Large Language Models for Traffic and Transportation Research: Methodologies, State of the Art, and Future Opportunities

The rapid rise of Large Language Models (LLMs) is transforming traffic and transportation research, with significant advancements emerging between the years 2023 and 2025 -- a period marked by the inception and swift growth of adopting and adapting LLMs for various traffic and transportation applications. However, despite these significant advancements, a systematic review and synthesis of the existing studies remain lacking. To address this gap, this paper provides a comprehensive review of the methodologies and applications of LLMs in traffic and transportation, highlighting their ability to process unstructured textual data to advance transportation research. We explore key applications, including autonomous driving, travel behavior prediction, and general transportation-related queries, alongside methodologies such as zero- or few-shot learning, prompt engineering, and fine-tuning. Our analysis identifies critical research gaps. From the methodological perspective, many research gaps can be addressed by integrating LLMs with existing tools and refining LLM architectures. From the application perspective, we identify numerous opportunities for LLMs to tackle a variety of traffic and transportation challenges, building upon existing research. By synthesizing these findings, this review not only clarifies the current state of LLM adoption and adaptation in traffic and transportation but also proposes future research directions, paving the way for smarter and more sustainable transportation systems.

==> Application/ADbackup.tex <==
Traffic research refers to the dynamic flow and movement of vehicles, pedestrians, and other entities within a transportation network. It focuses on the operational aspects of mobility, including real-time interactions between road users, traffic flow optimization, and accident prevention. Unlike the broader study of transportation, which encompasses infrastructure development and policy, traffic studies emphasize the immediate and localized behavior of entities within existing systems.

In this section, we explore the role of advanced technologies, particularly Large Language Models (LLMs), in transforming traffic systems. Key areas of focus include autonomous driving, accident analysis, emergency management, traffic safety, and traffic forecasting. These applications demonstrate how LLMs can enhance decision-making, improve system efficiency, and address complex challenges in modern traffic networks.

\subsubsection{Autonomous Driving (yejia and xi)}

Autonomous driving (AD) is an emerging technology with the potential to revolutionize intelligent transportation systems by improving safety and enhancing mobility \autocite{kuo2023public}. Although autonomous driving intersects both traffic and transportation domains, it aligns more closely with traffic systems. This is because autonomous driving primarily deals with the operational aspects of vehicle movement, real-time decision-making, and interaction with other road users (vehicles, pedestrians, cyclists) within existing transportation infrastructure. It is therefore classified as a part of traffic studies in our survey.

The development of these core AD components has seen significant technological evolution. Initially, rule-based and optimization-based methods \autocite{yuan2024evolutionary} dominated the field. While these traditional approaches produce reliable and interpretable results, they often struggle to handle complex and novel scenarios \cite{aksjonov2021rule,guanetti2018control}. The field then progressed to learning-based methods, such as reinforcement learning \autocite{yan2022reinforcement}, which demonstrated improved accuracy in handling complex scenarios and making predictions. However, these methods face two key limitations: their "black box" nature makes interactions between vehicles and surroundings less interpretable, and they struggle with long-tail scenarios involving rare or unexpected events.

Most recently, Large Language Models (LLMs) have emerged as a promising advancement in autonomous driving development. Several comprehensive surveys (e.g., \cite{yang2023llm4drive, li2024large, cui2024survey, zhou2024vision}) \textcolor{blue}{[YM: may need to delete]} have documented LLMs' contributions to autonomous driving. LLMs present distinct advantages over conventional approaches: they better handle long-tail scenarios, enable sophisticated reasoning and knowledge accumulation from expert inputs, and can interpret human intentions and emotions. Their adaptability through fine-tuning allows for continuous performance improvements.

However, the application of LLMs in autonomous driving isn't without challenges. Key concerns include the transparency and interpretability of LLM decision-making processes in autonomous vehicles, and the need to ensure robustness against potential misuse. This section will examine these aspects in detail, covering the state-of-the-art in autonomous driving components, popular frameworks, and foundational models, before analyzing both the benefits and challenges of LLM integration in autonomous driving.

At the core of autonomous driving (AD) are four key components: perception, action planning, decision-making, and control systems. These elements work together to implement autonomous driving capabilities: perception systems interpret the surrounding environment, action planning determines the appropriate driving strategy, decision-making selects specific actions based on the interpreted environment and planned strategy, and control systems execute these decisions through vehicle operations. In this section, we introduce these four important aspects. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Application//Figures/AD.png}
    \caption{Autonomous Driving Framework (Need to be revised)}
    \label{fig:AD}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Application//Figures/longtail.png}
    \caption{Human driving vs. AD \ym{need to redraw}}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{Application//Figures/advancementinAD_new.png}
    \caption{Advancements in Autonomous Driving}
    \label{fig:enter-label}
\end{figure}

{End-to-end driving(novel) or closed-loop(traditional)} perception, decision-making, planning, control, reflection/feedback
\cite{pan2024vlp}enhanced VLP to improve the end-to-end autonomous driving capabilities.\cite{azarafza2024hybrid}, \cite{wang2024bevgpt}, \cite{chen2024driving} \ym{[YM: what is this, not finished]}


\textbf{Perception using LLM}

Perception is a critical process in autonomous driving, where the vehicle collects, processes, and interprets data from its environment to develop an understanding of its surroundings. This involves tasks such as object recognition, environmental mapping, and situational awareness, which are typically powered by data from sensors like LiDAR, cameras, and radar. LLMs have been integrated into perception systems to enhance the accuracy and efficiency of these tasks. They contribute by improving object detection and classification algorithms, enabling more sophisticated environment mapping, and refining the vehicle’s ability to understand complex, dynamic environments. Research in this area has demonstrated that LLMs can significantly augment traditional perception systems, offering a higher degree of contextual understanding and adaptability.

(xi) Within the perception module, object detection is an essential subtask that allows the AV to identify and locate relevant objects on the road — such as vehicles, pedestrians, cyclists, and traffic signs.  Researchers have applied and proposed LLMs to enhance object detection, especially focusing on challenging "corner case" scenarios. \cite{liu2023text} introduces a zero-shot detection approach using the GroundingDINO model, which leverages text prompts to identify objects without prior training, allowing the vehicle to recognize unexpected items in real-world settings. \cite{li2024automated} presents CODA-LM, a benchmark framework for evaluating large vision-language models (LVLMs) in handling rare, complex events, demonstrating the importance of combining visual and language models to enhance the general perception of corner cases. Similarly, the integration of Large Language Models (LLMs) is explored to augment scene understanding and object detection, using LLMs to provide reasoning capabilities that improve safety in uncertain driving conditions (\cite{wang2023empowering}). Furthermore, \cite{xiao2024multimodal} the Multimodal-Enhanced Objectness Learner (MENOL) leverages both visual and text data to improve the detection of unknown classes, addressing the challenges of novel object detection in autonomous driving. These approaches collectively illustrate the evolution of object detection techniques towards more robust, adaptable systems capable of perceiving complex environments, ultimately enhancing the reliability and safety of autonomous vehicles. \ym{[ym;very monotonic. Have not explained what is corner case scenarios.]}

(yejia, 3d perception, spatial and temporal) The reasoning ability is essential for LLM agents to make appropriate understanding of driving scenes and decision while driving, especially when ego vehicles interacting with environments and other participants. However, the spatial reasoning capabilities can be limited by the 2D visual input from camera. To integrate 3D information, \cite{wang2024omnidrive} proposed the OmniDrive that starts with a 3D MLLM architecture that converts visual presentation into 3D. Better scene understanding can be achieved and help AD make informed driving decisions. Accurately perceiving intentions from other road participants is another challenge that impedes the adoption of LLM. To tackle the challenge, \cite{wen2024road} leverage the visual language model, which is GPT-4V(ision), to investigate the long-tail scene and intentions of other road participants. However, the authors mentioned that the lack of 3D spatial reasoning capabilities make the GPT-4V struggle with precise judgments. Overall, the integration of 3D information can improve the spatial reasoning capability, as well as the safer operation. 
(yejia, perception, scene, image sequence) The SOTA MLLMs, such GPT-4V, have demonstrated unprecedented capabilities in image understanding and generating image/context contents \cite{yang2024harnessing}. However, these powerful models have not been tested for scene (sequence of images) reasoning and understanding. According to extensive experiments carried by \cite{sreeram2024probing}, while the SOTA MLLMs demonstrate robust proficiency in understanding individual images, they struggle to synthesis a coherent narrative or logic across a sequence of frames depicting dynamic behaviors. For instance, the accuracies for GPT-4V to predict behaviors like moving forward or backward, accelerating or decelerating are as surprisingly low as 50 percent and 35 percent. And GPT-4V failed heavily in identifying speeding cars. From these perspective, it remains a huge gaps for MLLLMs to understand dynamic behaviors, which may be highly correlated with the 3D information and identifying driving intentions of other road participants.



\textbf{Decision-Making using LLM}

Decision-making is another critical aspect of autonomous driving, involving the selection of appropriate actions based on information provided by the perception system. This process requires analyzing the environment, predicting potential outcomes, and determining the best course of action while considering factors such as safety, legality, efficiency, and passenger comfort. LLMs have been employed to enhance decision-making processes by leveraging environmental data and generating more sophisticated action plans \autocite{azarafza2024hybrid}. Their ability to process and analyze large volumes of data quickly allows for real-time decision-making that is both more informed and responsive to the complexities of the driving environment, such as unusual scenarios.
Based on the SOTA autonomous driving applications, most of them involve the prompt engineering methods that take the information from perception and textual description of the situation awareness and human intentions. More specific, the SOTA mentioned several major components, they are human instruction, perception, reflection and reasoning, and memory module. Human instruction serves as an option related to the level of human intervention or level of automation. The perception provides correct situation information, and the reasoning module can use the perception and experiences from memory module and scenarios descriptions, and decode the responses from LLMs to finish the decision-making process. Concurrently, the reflection module evaluates these decisions, identifying unsafe results, optional help from experts, and updates the revised experiences into memory module. There are many SOTA leverage similar framework, such as DILU\cite{wen2023dilu}, DRIVELLM\cite{cui2023drivellm}, DriveLikeAHuman\cite{fu2024drive}, and DriveGPT4\cite{xu2024drivegpt4}, the DriveGPT4 can generate the low-level control signal, such as vehicle speed and turning angle, and \cite{cui2024drive}
The LLMs applications are not limited to self-driving, it also consider interaction with infrastructure, such as The Mult-trask decision-making generative pre-trained transformer\cite{liu2023mtd}. and are explored in mining industry, such as\cite{li2024miningllm}.
However, the limitation of computing power and network communication condition can be a significant barrier for calling online LLMs. To leverage the capabilities of LLMs, the onboard deployment of LLMs is in need. \cite{wang2024drive} proposed a fine-tuned LLaMA-7B to substitute the online MLLMs to generate driving tasks. In this smaller-sized onboard LLM, the authors used training set consisting of instructions, scenarios, and human-annotated driving tasks. And the LoRA method is widely used in onboard solutions to fine tune the onboard LLMs with the advantages of reduced cost and faster training speed. However, the current limitations should not be ignored, including the slow generation speed that does not meet the real-time requirements. The capabilities of onboard solution should be broaden to more complex and novel scenarios. \textcolor{blue}{[YM: there are many grammar errors in this paragraph]}

\subsubsection{Expanding Onboard Solution Capabilities}

To address the aforementioned limitations, it is imperative to explore methods that enhance the speed and efficiency of onboard solutions. One promising avenue is the utilization of advanced hardware accelerators. These devices, such as \ym{[YM: Is it halfway through here?]}
\textbf{Trajectory planning using LLM}
Trajectory planning is a follow up procedure after the drive agent make a driving decision, achieving the closed-loop driving task. The AD vehicles follow the planned trajectories with the consideration of the ride comfort, driving efficiency and driving safety.  However, existing motion planners predominantly leverage heuristic methods to forecast driving trajectories, yet these approaches show limited generalization capabilities in the face of novel and unseen driving scenarios. \cite{mao2023gpt} proposed the GPT-Driver to generate the driving trajectories through a language description of coordinate position. There is a research claimed that the trajectories prediction can be improved by integrating pre-trained language model \cite{keysan2023can}. And the refined trajectories prediction can be further improved in a closed-loop framework. \cite{fu2024limsim++} proposed a closed-loop simulation platform for deploying MLLMs in AD, which was LimSim++. This platform can convert the decisions from MLLMs into vehicle trajectories. Then the evaluation module quantifies and assesses the vehicle behavior decisions made by MLLMs based on the analysis of vehicle trajectories. With the evaluation, LimSim++ employed the reflection and memory module to enhance the driver agent's performance, which further feedback in to MLLMs to refine the decision accuracy. Thus, the refined reasoning outcomes will act as few-shot instances to aid MLLMs in the subsequent decision-making process.  \textcolor{blue}{[YM: Need to have the results of these works]}(results, compared to baseline)
Apart from doing trajectory planning for ego-vehicle, \cite{lan2024traj} proposed the Traj-LLM to predict the future trajectories of dynamic traffic actors without explicit prompt engineering to generate future motion from agents' past/observed trajectories and semantics and revealed a 7 percent to 30 percent improvement over several trajectory prediction benchmarks. Similarly, \cite{xia2024language} proposed InteractTraj to generate interactive traffic trajectories, achieving 16 percent improvements over other methods. These efforts highlight the importance that the efficient and safe trajectory planning should consider surrounding vehicles' movement and the interactions. 



\textbf{Vehicle control using LLM}
Vehicle control involves generating actuation signals for steering angle, acceleration, deceleration, and distance management, which are guided by the outcomes of perception, decision-making, and planning processes. In the context of LLM-controlled vehicles, the accuracy of these systems in perceiving and making decisions directly affects the smoothness and safety of the vehicle’s maneuvers, potentially causing user discomfort or shock due to unexpected behavior. Research, such as reinforcement learning from human feedback (RLHF), has been explored as a key strategy for fine-tuning LLM systems to better align with human driving preferences, as highlighted by \autocite{stiennon2020learning} and\autocite{rafailov2024direct} . In this approach, LLMs are trained to follow user instructions for vehicle control tasks, such as adjusting steering or speed. For instance, \cite{cui2024drive} leveraged GPT-4 to receive human input and make driving decisions based on perception, localization, and in-cabin monitoring, integrating human interaction and feedback to enhance decision-making accuracy. With advances in LLMs, they are increasingly capable of handling end-to-end driving tasks with minimal or no human intervention. \cite{chen2024driving} demonstrated the effectiveness of LLMs in generating accurate control actions through a driving question-answering framework, which combines reasoning and perception to execute appropriate vehicle maneuvers, paving the way for more autonomous and explainable vehicle control systems.

\textbf{Benefits analysis} ## move to future direction

Evaluation
Reasoning is defined as ability to draw inference on new or known information\autocite{honderich2005}. LLMs have shown the traits, drawing accurate conclusion by applying logic to new or previously unseen data sample. This capability is frequently referred as zero-shot or one-shot learning\autocite{brown2020language}. However, the accuracy of zero-shot learning requires evaluation and reflection to improve the performance.
Evaluation is a crucial part in the AD system to improve the AD performance, including, safety, efficiency, and passenger comfort. This can be referred as a learning process to build the robustness AD system. In the reviewed literature, it can be the reflection module, \cite{wen2023dilu} integrated the reflection module that takes recorded decisions generated by LLMs from closed-loop driving tasks as input and utilized a summarization and correction module  to identify safe and unsafe decision. These correction procedure finally generate historical driving experience and enrich the memory module.  There is other research employed the experts to give feedback for the generated or simulated driving tasks\autocite{wang2023chatgpt}. The proposed LLMs can be trained with minimal labeled data to perform driving-related tasks, where it usually referred as few-shot learning. Together with the experts' input, this research enhances the success rate.
The experiment conducted by \cite{wen2023dilu} shows an improved success rate when performing driving tasks. A summarized evaluation metrics are provided below.

Task-specific metric
Instruction following accuracy: evaluate the accuracy of instruction interpretation and execution. Reasoning chain of thought can be checked.
Response time: evaluate how quickly the LLM processes command and respond, as delay could impact driving safety.
Contextual understanding: 

Safety and reliability metrics
Critical error rate: evaluate the frequency of severe mistakes
Collision and Near-miss rate: assess the occurrence of collisions and near misses when interacting with other vehicles, pedestrians, and objects.
False positives/negatives in hazard detection: evaluate the ability to correctly interpret alerts about potential hazards and avoid false positives that lead to unnecessary actions, like brake and lane change.

Comfort: evaluate the model's ability to provide comfortatble driving experience.






{Peer review concern}

By analyzing open reviews to some literature \autocite{openreview2024, openreview2024b,openreview2024c}, the reviewers' concern can be summarized:
1. With the accumulating the real-world situations, such as corner cases, which may introduce the complexity. The scalability of the SOTA methods should be further discussed and the model's ability to provide timely response should be investigated. The few-shot learning methods might increase the response time and require higher computation resources.
2. Thoroughly evaluation is required. SOTA frameworks employed different evaluation metrics on different datasets. The comprehensive evaluation standards and metrics are needed for efficient comparison. Different testing scenario and datasets are utilized in different SOTA methods, which make it hard to compare the advantages of different models and has unpredictable gaps between simulation and real-world scenarios. Thus, a comprehensive and updating test scenarios and dataset is prefered for developing and improving novel applications.
3. The model backbones, such as GPT, keep revolving quickly. The model advancements should be discussed to understand the requirement, such reasoning accuracy and timely respond and knowledge, convergence.
4. The inherent latency issue due to reliance on API calls to LLM is still a concern.
5. The consistency  of LLM results should be further discussed with respect to the advancements of LLMs.
6. How is the interaction between other road users to the LLM agents?
7. A common question surrounding LLM-based agents is their trustworthiness. For safety-critical applications such as autonomous driving, the safety requirements are significantly higher than those for tasks like question-answering or code generation.
8. The logical reasoning ability of LLM should be investigated. 


{Conclusion} ## mention gaps and future direction


\paragraph{Gaps and future direction (yejia)}
\textcolor{blue}{[YM: may move to future research direction section]}
State-of-the-art research often utilizes visual input modalities and prompt generators to interact with large language models (LLMs) in autonomous driving systems. However, the spatial and temporal relationships between the ego vehicle and its surrounding environment require further exploration. While some studies attempt to enhance scene understanding by using video inputs or converting 2D images into 3D spatial information, the accuracy and capabilities of these approaches still need to be validated and expanded. Additionally, research has shown that relying solely on static images for decision-making and scene understanding in LLMs presents challenges. The accuracy of correctly interpreting such scenes is relatively low, highlighting the need for better fine-tuning of the perception process to improve LLM performance.Another significant issue is whether to deploy online LLMs, locally deployed onboard LLMs (such as LLaMa), or a hybrid approach. Online LLMs have the advantage of continuous learning from novel scenarios, while onboard LLMs offer benefits like reduced reliance on network connectivity, lower computational demands, and faster decision-making. A hybrid solution may balance these trade-offs, combining the strengths of both approaches to enhance the overall system’s robustness and efficiency.

\begin{table}[htbp]
\tiny
\centering
\begin{threeparttable}
\caption{LLMs in Autonomous Driving}
\begin{tabular}{>{\raggedright}p{2cm} l>{\raggedright}p{2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2cm} >{\raggedright}p{2.2cm} >{\raggedright\arraybackslash}p{2.2cm}}
\toprule
\rowcolor{gray!20}
\textbf{Literature}  &Model name& \textbf{Model Backbone} & \textbf{Input} & \textbf{Output} & \textbf{Modality} & \textbf{Task} & \textbf{Data Source} \\
\midrule
 \cite{wen2023dilu}  &DiLu& GPT-3.5 and GPT4.0 & System prompts, textual description, and few-shot experience & driving action & Text & decision making & drone-based vehicle trajectories dataset \cite{zheng2024citysim}\\
 \cite{cui2023drivellm}  && GPT-3.5 & image, location, vehicle state, weather, and experience & driving action & Text and image & Perception and decision making & https://github.com/DriveLLM/DriveLLM \\
 
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
    \item EV: Electric Vehicle
\end{tablenotes}
\end{threeparttable}
\end{table}




==> Application/IndustryApplication.tex <==
\subsection{Industry Application}
\label{subsection:IndustryApplication}
The implementation of LLMs in industrial logistics and transportation has shown distinct characteristics in different regions, where different technological approaches and business priorities have shaped their development.

Traditional supply chain forecasting relies on structured historical sales data and statistical models, which often struggle to incorporate external factors like market trends or consumer sentiment. In contrast, LLMs excel at processing unstructured data—such as social media discussions, product reviews, and news articles—to identify hidden demand signals. By synthesizing these diverse inputs, LLMs enhance the accuracy of demand predictions and enable dynamic replenishment planning. Cainiao’s Tianji π leverages this capability to analyze multi-source data, automating inventory optimization and mitigating risks like overstocking or stockouts. Its adaptability allows customization across industries, from retail to manufacturing, demonstrating how LLMs bridge the gap between static historical analysis and real-time market responsiveness.

Conventional logistics systems depend on manual address verification and GPS coordinates, which falter in regions with informal or landmark-based addressing. LLMs, trained on vast datasets of location-specific patterns, can interpret ambiguous addresses, predict geo-coordinates, and standardize formats dynamically.
In India, Ecom Express’s Bulls.ai addresses last-mile challenges by decoding vague addresses (e.g., “near the temple”) into precise locations. Integrated into real-time APIs, the model not only corrects errors but also supports route optimization and fraud detection, showcasing LLMs’ role in transforming chaotic delivery landscapes into structured workflows.

Automated customer service relies on scripted responses and rigid workflows, limiting adaptability to unique queries. LLMs enhance these interactions by extracting context from conversations, generating summaries, and providing real-time guidance. For employees, they act as on-demand knowledge bases, reducing reliance on manual training. SF Express’s Fengyu streamlines customer support by auto-generating service summaries with high accuracy. For delivery personnel, it answers complex queries (e.g., customs rules or packaging guidelines), effectively acting as a digital co-pilot. This dual functionality underscores LLMs’ ability to augment both customer and employee experiences.

LLMs like Walmart’s BARD and Maersk’s Maersk Pulse are deployed to preempt supply chain disruptions. By analyzing unstructured data—weather reports, social media, and news—these models identify risks such as port congestion or weather delays. Their ability to synthesize natural language data enables proactive rerouting, inventory adjustments, and stakeholder communication, positioning them as critical tools for enhancing supply chain resilience in volatile environments.

Legacy supply chain collaboration often suffers from fragmented communication and data silos. LLMs facilitate unified platforms where partners share insights, forecasts, and operational data, translating complex information into actionable steps for all stakeholders. For example, Samsung’s AI One harmonizes data from suppliers, distributors, and manufacturers to identify bottlenecks and synchronize production schedules. This collaborative framework highlights LLMs’ capacity to break down silos and foster end-to-end supply chain transparency.

In conclusion, the adoption of LLMs in logistics and delivery services represents a significant leap forward in the industry's technological capabilities. As companies continue to innovate and refine these systems, we can expect to see even more sophisticated applications that further streamline operations, reduce costs, and enhance customer satisfaction across the global transportation industry.

% Other applications: packaging, sourcing and procurement, scheduling, predictive maintenance, warehousing, distribution network design, Supply chain risk management, sustainability

% The implementation of LLMs in industrial logistics and transportation has shown distinct characteristics in different regions, particularly in the United States and China, where different technological approaches and business priorities have shaped their development.

% In the US market, AWS's generative AI-powered data onboarding system, built on Amazon Bedrock, exemplifies this approach by automating the transformation and integration of supply chain data. The system employs LLMs to automatically map headers from input files to AWS Supply Chain's canonical data model, significantly reducing manual data processing efforts. This solution particularly benefits organizations dealing with multiple data sources and formats, enabling faster data-driven decision-making in supply chain operations.

% The US market has also seen significant development in LLM-powered AI agents for operational coordination. These systems handle complex communication workflows, including automated processing of RFQs and documentation, multi-stakeholder coordination, real-time response generation, integration with existing database systems, and automated cost calculation and quote generation. The implementation of these AI agents has particularly benefited the handling of complex freight coordination tasks, where multiple parties across different time zones and regulatory environments must interact seamlessly.

% China's approach to LLM implementation in logistics shows a stronger focus on comprehensive, integrated systems that combine industry-specific knowledge with general language capabilities. JD.com's Yanxi LLM represents this approach, with its unique 70-30 split between general and industry-specific data. This specialized model demonstrates superior performance in warehouse layout optimization, peak season operations planning, marketing content generation, and intelligent customer service. The model's deep understanding of retail, healthcare, logistics, and finance sectors enables it to provide actionable recommendations for complex operational challenges, such as optimizing warehouse operations during high-demand periods like Singles' Day.

% SF Express's Fengzhi LLM showcases an innovative hybrid approach, combining large language models with traditional smaller models to create a comprehensive supply chain intelligent agent. The system excels in sales forecasting, route optimization, and packaging recommendations. Through its implementation of Reinforcement Learning from Human Feedback (RLHF) fine-tuning techniques, Fengzhi continuously improves its performance based on user adjustments and business preferences, creating a more adaptive and responsive logistics solution.

% Cainiao's Tianji system, developed in collaboration with Alibaba DAMO Academy, represents another significant advancement in Chinese logistics AI. The system integrates deep learning algorithms with vast logistics data to optimize transport routes, warehouse operations, and resource allocation. Tianji's comprehensive approach extends beyond traditional optimization to explore cutting-edge technologies such as autonomous vehicles and delivery robots, positioning it at the forefront of future logistics solutions.

% These implementations in both regions demonstrate the versatility and effectiveness of LLMs in logistics operations. While US applications tend to focus on specific operational challenges and data integration, Chinese implementations often take a more holistic approach, integrating LLMs into comprehensive supply chain management systems. Both approaches have proven successful in their respective markets, showing how LLMs can be adapted to different business environments and operational requirements.

% The use of LLMs in these diverse scenarios highlights several key advantages:

% \textbf{Data Integration}: LLMs can effectively combine general knowledge with industry-specific data, as seen in JD.com's Yanxi model, enabling more accurate and contextually relevant decision-making.

% \textbf{Multi-faceted Optimization}: From Amazon's supply chain optimization to menu categorization (DoorDash), LLMs are proving valuable across various aspects of logistics and delivery services.

% \textbf{Continuous Learning}: The incorporation of RLHF techniques, as demonstrated by SF Express's Fengzhi model, allows for ongoing improvement based on real-world feedback and business preferences.

% \textbf{Enhanced Customer Experience}: LLMs contribute to improved service quality, whether through more efficient deliveries (UPS) or better product descriptions and categorization (DoorDash).

% \textbf{Sustainability}: The optimization capabilities of these systems, particularly in route planning, contribute to reduced fuel consumption and lower carbon emissions.

% In conclusion, the adoption of LLMs in logistics and delivery services represents a significant leap forward in the industry's technological capabilities. As companies continue to innovate and refine these systems, we can expect to see even more sophisticated applications that further streamline operations, reduce costs, and enhance customer satisfaction across global supply chains.

==> Application/Safetybackup.tex <==
\subsubsection{Traffic Safety (Guanhao)}
\label{subsubsection1:TrafficSafety}
Traffic safety is a major concern globally, with millions of traffic accidents leading to fatalities, injuries, and economic losses. 

Traditional traffic safety analysis methods focus on statistical modeling, crash frequency analysis, and crash severity analysis, which provide essential insights into factors contributing to crashes \autocite{dong2014multivariate,mannering2014analytic,lord2010statistical}. However, these approaches face barriers, including the inability to capture nuanced, context-specific information embedded in unstructured data sources, like police reports and incident logs \autocite{kwayu2021data}. Consequently, many valuable insights remain inaccessible, as existing methods do not leverage advancements in data extraction and interpretation. This limitation restricts a comprehensive understanding of underlying causes and dynamic factors affecting road safety, highlighting the need for approaches capable of extracting, synthesizing, and analyzing the vast and varied data generated from traffic-related incidents. 

Leveraging advancements in LLMs offers a solution by enabling automated interpretation of unstructured text data which traditionally require manual processing and allows for deeper insights and more efficient analysis, making it feasible to process large volumes of complex, context-rich data. The application of LLMs in traffic safety builds on the foundational work in Natural Language Processing (NLP), starting with efforts to process and analyze unstructured traffic safety data.

\paragraph{Use of Natural Language processing}

Historically, traffic safety-related data, such as traffic volume and crash reports, relied heavily on structured formats from sensors, detectors, or human reports. While useful, this approach had clear limitations in terms of cost, coverage, and reliability.  
Natural Language Processing (NLP) has emerged as a powerful tool in traffic safety, particularly in addressing the limitations of traditional sensor-based systems. By transforming unstructured text data into structured formats, NLP allows for more comprehensive traffic monitoring and incident detection. For example, \cite{wang2017exploring} focused on converting unstructured textual data into structured spatial information to enhance accident location detection using NLP. This approach significantly reduces the time required for processing various types of unstructured data, such as crash reports, allowing traffic management systems to quickly access and analyze crucial information.

A major benefit of using NLP for traffic safety is that it can process a great amount of real-time, unstructured data enables better prediction and analysis of traffic conditions as well as more informed decision-making. Studies like \cite{sampath2023traffic} leveraged Twitter data to predict traffic congestion, showcasing how NLP can integrate social media activity with traffic patterns to anticipate potential issues in real time. Similarly, sentiment analysis has been employed to gauge public reaction to traffic incidents, adding a deeper layer of insight into traffic conditions and potential hazards. This predictive power of NLP has also been applied to optimize emergency responses, as shown in \cite{ceklic2022ambulance}, where NLP techniques were used to prioritize ambulance dispatches.

In addition to real-time detection and prediction, NLP complements traditional traffic management systems by filling gaps in sensor data. \cite{ali2021traffic} and \cite{wan2020empowering} illustrated how NLP can augment Intelligent Transportation Systems (ITS) by processing social media data to provide a more comprehensive view of traffic events. This integration of unstructured data sources with existing systems leads to a more efficient and responsive approach to traffic management, offering a promising direction for future traffic safety improvements.

\paragraph{Use of Large Language Models}

The recent integration of Large Language Models (LLMs) into traffic safety builds on the foundation laid by traditional NLP techniques, offering substantial improvements in how traffic data is processed and used for safety applications. LLMs, due to their scale and sophistication, are particularly adept at handling vast amounts of unstructured data, including accident reports, real-time traffic updates, and even multimodal inputs like images and sensor data. The primary focus of these applications is to improve automation, enhance real-time data processing, and advance predictive capabilities in traffic safety.

\textbf{Automation of complex data processing} A key contribution of LLMs is the automation of complex data processing tasks, particularly accident report generation and analysis. Previous NLP-based systems focused on structured data or manually entered reports, but LLMs, as demonstrated by models like TrafficSafetyGPT \autocite{zheng2023trafficsafetygpt}, have shown the ability to automatically extract essential information from unstructured data sources. By fine-tuning general-purpose models with domain-specific knowledge, such as accident reports and government guidelines, LLMs streamline the process of data extraction, imputation, and summarization. This capability not only saves time but also reduces human error, improving the overall efficiency of traffic management systems \autocite{zheng2023trafficsafetygpt,zheng2023chatgpt}.

\textbf{Integration of multimodal data} Another significant advancement of LLMs over traditional NLP models is that LLMS can integrate multimodal data. For example, models that integrate both visual and linguistic cues can now analyze traffic incidents in real time using data from various sources such as traffic cameras, weather reports, and textual accident descriptions \autocite{de2023llm}. This multi-source approach allows LLMs to create a more comprehensive understanding of traffic situations, enabling them to forecast accidents more accurately and assist in the deployment of real-time interventions. The fusion of text and image data, such as the work done using visual language models (VLMs) and deep probabilistic reasoning, demonstrates how LLMs can enhance decision-making in autonomous vehicle systems and real-time traffic monitoring \autocite{de2023llm,zheng2023chatgpt}.

\textbf{Enhanced predictive analysis} Finally, the use of LLMs can further improve traffic prediction and proactive safety management. By analyzing complex datasets from various sources, LLMs can predict high-risk traffic conditions and accidents with greater accuracy than traditional statistical methods. Studies that apply models like BERT to predict accident types, or use GPT-based models to analyze real-time traffic conditions, show how these tools can improve traffic flow optimization and even assist in emergency response planning by prioritizing high-risk areas \autocite{baumler2024predicting,wang2024real}. This predictive capability is not limited to textual data but extends to larger traffic datasets, allowing LLMs to serve as central components in intelligent traffic management systems that adapt in real time to emerging risks \autocite{wang2024real}.

\paragraph{Accidents Analysis}
Accident analysis has traditionally faced significant challenges due to the rarity of accidents, whether man-made or natural, making them difficult subjects of study. The vast majority of traffic data reflects regular conditions, with accidents being outliers that are not easily modeled. This imbalance creates a challenge for researchers trying to predict and prevent crashes. The application of LLMs in this context can help address this issue by augmenting accident datasets, effectively enabling scenario generation and simulation. For example, \cite{Chang2024LLMScenario} applies scenario engineering of various tokens (scenario, instruction, and experience) to output scenarios including vehicle trajectories, lane changes, and risk analysis under challenging edge scenarios that do not frequently occur in daily observations. LLMs provide enhanced modeling capabilities by using synthetic data to complement real-world records, improving the robustness of safety research in low-frequency, high-impact events such as traffic accidents. 

A further gap in accident analysis with traditional methods lies in the limited consideration of the complex interactions between various contributing factors in crash frequency models. Traditional models often fail to fully account for the complex dynamics that lead to certain crash events, resulting in a constrained understanding of the mechanisms at play. This limitation restricts the potential for comprehensive preventive measures. By incorporating LLMs, which can process and model complex, multi-dimensional data, researchers can better capture these interactions, leading to more accurate predictions and more effective interventions aimed at reducing traffic accidents. While traditional NLP methods approach accident analysis with a lumped estimate of severity or quantified loss \autocite{Krause2019NewInsights, Kwayu2022AutomaticTopics}, recent applications of vision language model (VLM) allow multi-dimensional, detailed account of various contributing factors of the players in an accident. For example, \cite{Xuan_2024_CVPR} applies segment extraction and dynamic prompt segmentation on video inputs to generate detailed captions of pedestrian behavior, vehicle behavior, road conditions, weather, and other contextual traffic information. Similarly, \cite{Wang2023AccidentGPT} developed a V2X-perception architecture to integrate inputs from panoramic multi-camera views and road devices to create a comprehensive understanding of the environment. 

In the decoding phase, LLM has also been applied to enhance the interpretation of the accident. With scenarios generated, LLMs can be applied to infer accident severity \autocite{Zhen2024LeveragingLLM}. The authors incorporate techniques such as Chain-of-Thought (CoT) reasoning and Prompt Engineering (PE) to guide these models in analyzing crash causes and severity outcomes. Although without comparison with traditional methods, the results suggest LLMs have very good reasoning capabilities, transparency, and performance. The other stream of research aims to predict traffic crash outcomes based on generated scenarios and communicate it with first responders, improving the speed of response \autocite{Fan2024LearningCrashes}. 

==> Application/TrafficForecasting_backup.tex <==
\subsubsection{Traffic Forecasting (Tong)}
\label{subsubsection:TrafficForecasting}
Traffic forecasting is essential for improving transportation systems by enabling better traffic management, reducing congestion, and optimizing infrastructure efficiency \autocite{liu2024end}. Accurate predictions support informed decision-making for both transportation agencies and users, whether for route planning or emergency response \autocite{liu2024heterogeneous}. Key metrics such as traffic volume, speed, travel time, and congestion levels can all benefit from the insights provided by traffic data. The application of LLMs in traffic flow forecasting leverages foundational techniques from NLP to incorporate textual data and predict spatial-temporal traffic flow series.

\paragraph{Traffic forecasting using NLP}

While traditional traffic flow prediction methods have been explored across many dimensions using various data sources, recent advances have integrated Natural Language Processing (NLP) to derive traffic-related insights from textual data, such as social media or news reports. NLP offers a new layer of information by analyzing contextual content related to traffic, weather, and human behavior. For example, \cite{essien2021deep} proposes a deep learning model that combines information extracted from tweet messages with traffic and weather data. By integrating real-time information from social media with traditional traffic and weather datasets, the model demonstrates how diverse data sources can enhance the accuracy of traffic predictions. Moreover, it is essential to develop a flexible and comprehensive framework that can predict long-term, context-aware traffic conditions for public users and transportation agencies. For instance, \cite{tsai2022traffic} addresses the gap in robust long-term traffic forecasting by incorporating social media features into predictive models.

In conclusion, the incorporation of NLP and textual data into traffic flow prediction opens new avenues for research, providing richer and more comprehensive datasets. By leveraging these innovations, we can create predictive models that are not only more accurate but also adaptable to the complexities of real-world traffic dynamics.

\paragraph{Traffic forecasting using LLM}

Recent advances in machine learning and artificial intelligence have opened up transformative opportunities for research in travel behavior and mobility modeling. In this context, the following studies provide valuable insights into the application of NLP and LLMs for understanding and predicting various aspects of human mobility. Specifically, the application of LLMs in traffic flow forecasting can be categorized into three key areas: traffic flow prediction, traffic flow data imputation, and traffic flow reasoning.

\begin{table}[htbp]
\label{tab:trafficForecasting}
\tiny
\centering
\begin{threeparttable}
\caption{Traffic Flow Forecasting}
\begin{tabular}{>{\raggedright}p{2cm} >{\raggedright}p{2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2cm} >{\raggedright}p{2.2cm} >{\raggedright\arraybackslash}p{2.2cm}}
\toprule
\rowcolor{gray!20}
\textbf{Literature} & \textbf{Model Backbone} & \textbf{Input} & \textbf{Output} & \textbf{Modality} & \textbf{Task} & \textbf{Data Source} \\
\midrule
 \cite{ren2024tpllm}& GPT 2 & Traffic flow series + Graph & Future traffic flow & Quantity & Traffic flow prediction & PeMS dataset \\
 \cite{liu2024spatial}& GPT 2, Llama2 & Traffic flow series + Graph & Future traffic flow & Quantity & Traffic flow prediction & NYCTaxi, CHBike\\
 \cite{jin2021trafficbert}& BERT & Traffic flow series + Weekday information & Future traffic flow & Quantity & Traffic flow prediction & PeMS \& METR-LA dataset \\
 \cite{huang2024enhancing} & GPT  & Traffic flow series + Semantic Information & Future traffic flow & Text \& Quantity & Traffic flow prediction & NYC Bike Share data \\
 \cite{zhang2024semantic} & Sentence Transformers & Incomplete traffic flow series + Semantic information & Imputed traffic data & Text \& quantity & Traffic data imputation & PeMS dataset\\
 \cite{wang2024traffic} & GPT 4 & Network-wide mobility info + Prompt & SQL queries + interpretations & Text \& quantity & Traffic flow reasoning & Network-wide mobility database\\
 \cite{guo2024explainable} & Llama2 & Traffic flow series + Graph & Explanation of link traffic flow & Text \& quantity & Traffic flow reasoning & LargeST dataset, OpenStreet, NOAA\\
 \cite{gebre2024ai} & GPT 4 & Traffic flow density + Prompt & Explanation of link traffic density & Text \& quantity & Traffic flow reasoning & NGSIM dataset \\ 
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table}

\textbf{Traffic flow prediction}
Traffic flow prediction aims to forecast future city-wide traffic patterns on specific road segments based on historical data. While LLMs are traditionally designed as autoregressive models for text generation, their architecture is not naturally aligned with the task of traffic flow prediction. However, a key similarity between language data and traffic flow data is their sequential nature. This opens up the potential for LLMs to be used as temporal feature extractors, even though they cannot directly generate time series data. By extracting temporal embeddings from sequential traffic data from LLMs \autocite{jin2021trafficbert}, these embeddings can be fed into other models such as GNNs or RNNs, to predict future traffic flow.

For instance, \cite{ren2024tpllm} proposes TPLLM, which uses pre-trained LLMs to leverage embedding from GNNs and CNNs to extract both temporal and spatial features. This approach captures sequential patterns while maintaining spatial dependencies in traffic networks. Furthermore, \cite{liu2024spatial} applies LLMs in traffic flow prediction by redefining time steps at each location as tokens. The model introduces a spatial-temporal embedding that learns both spatial locations and global temporal representations of these tokens, where each token has unified spatial and temporal information. \cite{huang2024enhancing} further explore the application of LLMs in traffic flow prediction by investigating two specific scenarios: regional-level and node-level traffic. In regional-level scenarios, textual information is represented as a node connected to the entire network, whereas in node-level scenarios, embeddings from the LLM act as additional nodes that connect specifically to corresponding traffic nodes.


Furthermore, the Low-Rank Adaptation (LoRA) fine-tuning approach is applied to the task of traffic flow prediction, thereby facilitating efficient learning and minimizing computational demands. \cite{ren2024tpllm} incorporate LoRA in the training of TPLLM, demonstrating that LoRA not only preserves the pre-existing knowledge embedded in the TPLLM but also enhances the model’s capability to make accurate predictions even with limited data.

\textcolor{blue}{[YM: may need to add]}
LLMs for Public Event Mobility Prediction
\cite{liang2023exploring} introduced LLM-MPE, a framework for predicting human mobility during public events using LLMs. Public events, such as concerts and sports games, often cause irregular surges in travel demand, posing challenges for traditional models that rely on regular patterns. LLM-MPE addresses these challenges by integrating unstructured textual event descriptions (e.g., concert details, artist popularity) with historical mobility data. Using Chain-of-Thought (CoT) prompting, the framework generates step-by-step reasoning for predictions, enhancing transparency and interpretability.

A case study of Barclays Center, NYC, demonstrates that LLM-MPE outperforms machine learning baselines like gradient-boosted decision trees (GBDT) and recurrent neural networks (RNNs). The inclusion of textual data improves prediction accuracy, while CoT prompting provides actionable insights for event organizers. However, the study identifies limitations such as high computational costs, inefficiency, and difficulty in modeling spatial relationships, highlighting areas for future research.

\textbf{Traffic data imputation}
Traffic data imputation is a crucial aspect of Intelligent Transportation Systems (ITS), particularly given the frequent challenge of large-scale missing data across road networks. Traditional methods often fail to account for the rich semantic information embedded in the spatial and temporal dynamics of traffic. With the advent of large language models (LLMs), however, there is now potential to harness semantic descriptions that capture these intricate relationships, offering a more nuanced understanding of traffic behavior. For instance, \cite{zhang2024semantic} utilizes GNNs and Sentence Transformer to perform large-scale traffic data imputation. This method utilizes sensor connectivity and semantic descriptions to fill in missing traffic data more effectively than traditional models. The integration of LLMs with other neural networks provide more accurate predictions by leveraging both semantic and spatial-temporal data, ultimately enhancing the precision of traffic data imputation in ITS.


\textbf{Traffic flow reasoning}
In the field of traffic flow forecasting, LLMs offer a significant advantage beyond traditional temporal and semantic embedding extraction. To illustrate, large language models excel at contextual understanding and reasoning in the traffic flow data. After predicting the traffic flow series, LLMs are also utilized to analyze the root causes of current conditions, identify bottlenecks, and offer management suggestions to alleviate these issues.

For instance, \cite{guo2024explainable} employs LLama2 with few-shot learning, using examples where traffic flow prediction and explanation are correctly aligned, to generate explanations after producing traffic flow predictions. \cite{wang2024traffic} takes a different approach by using GPT-4 to generate accurate SQL queries and natural language interpretations based on specific transportation tasks and scenarios, using Chain-of-Thought prompting. \cite{gebre2024ai} integrates Physics-informed neural networks with LLMs, allowing users to input multiple queries about traffic flow at specific locations and times, with GPT-4 providing human-like reasoning and explanations.

In summary, integrating LLMs into transportation flow forecasting offers significant advancements in real-time reasoning and management. LLMs serve three key roles: (1) LLMs interpret human prompts and generate SQL queries or code to extract relevant data; (2) LLMs serve as temporal and semantic information extractors, capturing the correlation between traffic flows; (3) LLMs interpret the traffic flow prediction results and provide suggestions to alleviate bottlenecks.
\ym{missing tables}

==> Application/aviationbackup.tex <==
\subsubsection{Aviation and Air Traffic Control (Ruili \& Xi)}
\label{subsubsection11111: Aviation and Air Traffic Control and UAVs}
\ym{[Significant problems in this section]}

Automation has long been embraced in the aviation and Air Traffic Control (ATC) areas, which have clearly defined processes; however, the environments are just as complex due to the need for accurate communication, real-time decisions, and human-machine interface challenges, combined with the noisy environment, accents, and strict regulatory compliance. These are increasingly being utilized in these domains to improve communication systems, facilitate decision-making, and increase the resilience of autonomic systems. In this section, we address and analyze recent progress with the application of LLMs to ATC and UAVs, and focus on how these technologies can be useful in overcoming these complex problems.

The application of LLMs has been widely studied in the field of Automatic Speech Recognition (ASR) in ATC. To resolve AGC, multi-block (multiple encoder-decoder providing separate contextual information) has been introduced in \cite{guo2021context} using an encoder-decoder architecture to embed contextual information into speech spectrograms to optimize ASR performance under complex ATC conditions. Likewise, \cite{zuluaga2022atco2} proposes a hybrid ASR architecture that handles ATC-specific communications with the ATCO2 corpus, successfully tackling challenges like diverse speaker accents and noise. Environmental Impact FTS \ym{[YM: what is FTS?]} is a family of high-performance models that use the powerful language understanding abilities of LLMs to enhance both the accuracy and stability of speech recognition, two key requirements in a critical situation such as ATC.

LLMs are also used in ATC for strategic decision support, apart from being used for speech recognition. \cite{abdulhak2024chatatc} leverages GPT-4 to produce strategic air traffic flow management (ATFM) recommendations using historical air traffic based database. It highlights the capability of LLMs to process vast amounts of aviation data and provide useful recommendations, improving the efficiency of air traffic management and alleviating the burden on human operators.

In ATC, LLMs are further used for predictive modeling. \cite{ma2024text} apply a transformer-based encoder to predict future air traffic levels based on flight callsign data. Forecasting the positional accuracy of orbital debris can help avoid airspace traffic congestion as air traffic controllers will have more time to manage such situations.

Data operated from LLM to reinforcement learning (RL) have also been exploited to improve autonomous flight control systems. The work of \cite{yang2024large} introduces a ChatGLM-6B model of six-degree-of-freedom (6-DOF) flight control that is integrated with LLM and RL. By incorporating data from multiple recent flights (up to a certain value) into a learning data set for KNN decision-making, this hybrid methodology brings context to standardized RL frameworks, leading to multiple low-cost flight maneuvers. This integration aids the autonomous systems to handle specific intricate flight scenarios and improves their real-time adaptability, proving advantageous in training and operational use cases.

In the case of UAVs, LLMs have bedrocked the innovation of navigation and communication systems. The model presented in \cite{liu2023aerialvln} understands natural language commands with visual inputs to help deploy a UAV in a specific target. With data shows up to 2023,Oct.
It is easy for user to control the UAV as the LLMs are csan and ease communication whether they are loss of line of sight or far from the range available. One such work that addresses this issue is \cite{carranza2023need}, which uses a custom LLM to allow UAVs to understand generative text-based instructions, providing a higher degree of interpretability and level of control during human-drone interactions. Likewise, \cite{chen2023typefly} makes use of LLMs to create an arbitrary flight path for UAVs from simplified text commands, enabling quick and precise deployment without manual control. These applications are indicative of ways that LLMs enhance UAVs through increased intuitiveness in operation, supporting more widespread vertical application.

They are also used for creative and complex Unmanned Aerial Vehicle (UAV) coordination by leveraging Vision-Language Models (VLMs) with LLMs. \cite{pueyo2024clipswarm} introduces CLIPSwarm, a system where drones create complex formations in response to natural language prompts. This application showcase the potential of VLMs, which may direct dynamic UAV behaviors for artistic and entertainment applications, without having to instruct individual flights a priori.
Furthermore, LLMs can play a significant role in improving UAVs' situational awareness capabilities. building on this, work such as \cite{de2023semantic} makes use of GPT-4 to visually scene interpret, which provides a level of semantic understanding that can inform the UAVs navigation. The integration of LLMs offers UAVs the ability to operate in a more semantically informed manner by mapping descriptive linguistic information to the spatiotemporal nature of visual data, thus equipping UAVs with rich contextual knowledge that makes sense in dynamic and unknown environments. \cite{alves2022dress} also presents DRESS-ML, which is a domain-specific language using LLMs to characterize self-adaptive behaviors in UAVs. Such approaches allow UAVs to adapt their actions based on unexpected conditions, enhancing robustness and autarky in uncertain environments.
The summarized research also demonstrates how LLMs can generate textual analysis to help parse and simplify ATC regulation. \cite{jarry2024effectiveness} classifies ATFM regulations using GPT-3, facilitating the comprehension of regulatory texts for air traffic controllers. This ensures accountability and helps informed decision making on the regulatory side.
In general terms, based on this research, LLMs are bringing significant advancements on various fronts for ATC and UAV operations. For example, in ATC, LLMs are used to improve communication systems, early emergency detection, and ease regulatory compliance. For UAV applications, LLMs play a role in improving navigation, communication, and adaptability, resulting in more complex and varied applications. These include ATCSpeech (\cite{guo2021context}) and ATCO2 (\cite{zuluaga2022atco2}) for air traffic control and UAV-specific datasets for other aerial systems.


\begin{table}[htbp]
\label{tab:aviationAirTrafficControl}
\tiny
\centering
\begin{threeparttable}
\caption{Aviation and Air Traffic Control}
\begin{tabular}{>{\raggedright}p{2cm} >{\raggedright}p{2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2.2cm} >{\raggedright}p{2cm} >{\raggedright}p{2.2cm} >{\raggedright\arraybackslash}p{2.2cm}}
\toprule
\rowcolor{gray!20}
\textbf{Literature} & \textbf{Model Backbone} & \textbf{Input} & \textbf{Output} & \textbf{Modality} & \textbf{Task} & \textbf{Data Source} \\
\midrule
\cite{guo2021context} & Encoder-Decoder & Speech spectrograms + context & Transcribed speech & Audio + Text & Speech Recognition & ATCSpeech Corpus \\
\cite{zuluaga2022atco2} & Hybrid ASR & ATC voice communications & Text transcripts & Audio & ASR + NLU & ATCO2 Corpus \\
\cite{abdulhak2024chatatc} & GPT-4 & Historical air traffic data & ATFM suggestions & Text & Conversational ATFM Support & Historical ATC Data \\
\cite{ma2024text} & Transformer Encoder & Flight callsigns & Predicted flight counts & Text + Sequence & Traffic Flow Prediction & Flight Record Data \\
\cite{yang2024large} & ChatGLM-6B & State variables + commands & Flight control actions & Flight Control Data & RL for 6-DOF Control & Flight Simulations \\
\cite{pueyo2024clipswarm} & CLIP Vision-Language & Text prompts & Drone formations & Visual + Text & Drone Show Generation & Simulation Data \\
\cite{liu2023aerialvln} & Vision-Language Navigation & Visual scenes + commands & UAV navigation paths & Visual + Text & Vision-Language UAV Navigation & UAV Visual Dataset \\
\cite{carranza2023need} & Custom LLM & Text prompts & UAV responses & Text & UAV Communication & Custom Dataset \\
\cite{chen2023typefly} & Large Language Model & Text commands & Drone flight paths & Text & UAV Flight Control & Simulation Data \\
\cite{de2023semantic} & GPT-4 & Scene descriptions & Semantic scene understanding & Multimodal & Scene Analysis & UAV Scene Dataset \\
\cite{alves2022dress} & Domain-Specific Language & Scenario specs & Adaptive drone behaviors & Text & Self-Adaptive UAV Scenarios & Scenario-Based Data \\
\cite{jarry2024effectiveness} & GPT-3 & ATFM regulations & Categorized regulations & Text & Textual Analysis & ATFM Regulatory Data \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
    \item ATFM: Air Traffic Flow Management
    \item ATC: Air Traffic Control
    \item 6-DOF: Six Degrees of Freedom
\end{tablenotes}
\end{threeparttable}
\end{table}








==> FutureDirections/PeerReview.tex <==
\subsection{Peer Review Concerns}
\label{subsubsection:PeerReview}

By analyzing open reviews to some literature \autocite{openreview2024, openreview2024b,openreview2024c}, the reviewers' concern can be summarized:
1. With the accumulating the real-world situations, such as corner cases, which may introduce the complexity. The scalability of the SOTA methods should be further discussed and the model's ability to provide timely response should be investigated. The few-shot learning methods might increase the response time and require higher computation resources.
2. Thoroughly evaluation is required. SOTA frameworks employed different evaluation metrics on different datasets. The comprehensive evaluation standards and metrics are needed for efficient comparison. Different testing scenario and datasets are utilized in different SOTA methods, which make it hard to compare the advantages of different models and has unpredictable gaps between simulation and real-world scenarios. Thus, a comprehensive and updating test scenarios and dataset is prefered for developing and improving novel applications.
3. The model backbones, such as GPT, keep revolving quickly. The model advancements should be discussed to understand the requirement, such reasoning accuracy and timely respond and knowledge, convergence.
4. The inherent latency issue due to reliance on API calls to LLM is still a concern.
5. The consistency  of LLM results should be further discussed with respect to the advancements of LLMs.
6. How is the interaction between other road users to the LLM agents?
7. A common question surrounding LLM-based agents is their trustworthiness. For safety-critical applications such as autonomous driving, the safety requirements are significantly higher than those for tasks like question-answering or code generation.
8. The logical reasoning ability of LLM should be investigated. 

==> Method/Methodbackup.tex <==
\textcolor{blue}{Between six and nine months, a child typically starts to learn its language starting from the surrounding environment. A newborn is exposed to an overwhelming amount of linguistic input - parents talking, sibling chattering, TV sounds and even books they see. Initially, these exposures are noise. But gradually, through consistent exposure and the pattern recognition repertoire of infants' brain, the child begins to make sense of the sea of information.}

\textcolor{blue}{This remarkable process mirrors how LLMs learn, beginning with their data foundation. Just as children absorb massive amounts of language input during their formative years, LLMs begin their development with enormous text \textit{datasets}. The parallel extends to the processing mechanism: just as human sensory organs (eyes and ears) perform initial pre-processing of linguistic input before neural transmission, LLMs employ sophisticated \textit{pre-processing} techniques to transform raw text into processable tokens. The neural networks underlying LLMs mirror our brain's architectural principles, though in a simplified and artificial form.}

\textcolor{blue}{Research shows that children learn approximately 7-10 words daily through reading and exposure, accumulating thousands of words by adulthood. Similarly, LLMs process vast amounts of text during \textit{pretraining}, building their foundational knowledge. This learning process is guided by the "distributional hypothesis," which suggests that both children and LLMs can learn meaning through observing how words appear together in context, forming intricate patterns of understanding through repeated exposure and contextual learning.}

\textcolor{blue}{Knowledge acquisition follows a similar trajectory in both systems. Children progress from basic vocabulary to complex language understanding, much like how LLMs develop from basic pattern recognition to sophisticated language processing. After acquiring basic language ability, children begin to learn domain-specific knowledge, very much similar to that of \textit{post-training} procedures such as fine-tuning of LLMs. This specialization phase allows both human learners and artificial systems to develop expertise in specific areas while building upon their foundational language understanding.}

\textcolor{blue}{This acquired knowledge then transforms into practical application. Children eventually use their language knowledge for various purposes - asking questions, telling stories, expressing emotions, and engaging in complex dialogues. Similarly, LLMs can apply their learned patterns to diverse tasks ranging from summarization and question answering to text completion and translation under appropriate \textit{interaction techniques}. The versatility of both systems demonstrates how fundamental language understanding can adapt to serve numerous practical purposes.}

\textcolor{blue}{This section establishes the foundation for understanding LLMs in traffic and transportation applications. It encompasses the essential components: datasets, pre-processing techniques, model architectures, training methodologies, interaction approaches, evaluation metrics, and existing model implementations. The accompanying mind map (Figure \ref{fig:mindmap}) visualizes these interconnected elements of LLM technology, illustrating how each component contributes to the system's overall capabilities.} 

\begin{figure}[h]
\centering
\includegraphics[width=0.98\textwidth]{Method/Figures/llm_backgroud.png}
\caption{LLMs background}
\label{fig:mindmap}
\end{figure}



\subsection{Key Concepts of LLMs}

Text is a sequence of words or symbols, which, when combined, convey meaning. Each language has its own rules (grammar), structures (syntax), and vocabulary (words and their meanings), making the task of processing and interpreting text more complex than it may initially seem. Computers don’t inherently understand the meaning of words; they process text as sequences of characters or tokens. For a computer, understanding human language means finding ways to represent these sequences meaningfully, typically through numerical representations. \textcolor{blue}{These representations are then processed by deep neural architectures, which generate human-like textual responses. The Transformer, as one of the most recent deep neural network architectures, has become the foundation for modern LLMs due to its ability to capture complex language patterns and contextual relationships within and across sentences \autocite{vaswani2017attention}.} \\

In transformers, tokenization breaks text into smaller units (tokens) for structured processing, and positional encoding adds information about each token’s order enabling all tokens to be processed simultaneously. The attention mechanism in transformers lets each token focus on other relevant tokens, capturing context and dependencies across the sequence. Together, these components enable LLMs to effectively understand and generate complex language patterns.

\textcolor{blue}{In this section, we only briefly introduce important components, for a more comprehensive review of how Transformer architecture is designed, coded and implemented, we direct readers to a more comprehensive tutorials \autocite{hadi2023survey, kalyan2021ammus, huang2023advancing}.

\subsubsection{The Transformer}

\textcolor{blue}{The Transformer architecture represents a pivotal advancement in deep learning that has become the foundation for modern large language models. This architecture overcame the limitations of previous sequential processing approaches by introducing a mechanism for parallel processing and direct modeling of long-range dependencies. The Transformer consists of an encoder stack that processes input sequences and a decoder stack that generates output sequences, though modern variants may use only the encoder or decoder components. At its core, the architecture relies on three key components: the attention mechanism, which enables dynamic focus on relevant parts of the input; the tokenization process, which converts text into processable tokens; and positional encoding, which maintains sequential information. The following sections detail these components and their roles in enabling the remarkable capabilities of modern language models.}

\paragraph{Attention Mechanism}
\textcolor{blue}{[YM: maybe we should add how self attention is linked to decoder/encoder]}
The core technique in Transformer is the usage of self-attention~\autocite{vaswani2017attention}, which brings two advantages that enable scaling. First, the attention mechanism enables a better contextual understanding by allowing the model to attend to other tokens with a distance of $O(1)$. More importantly, different from recurrent neural networks that process sequences sequentially, attention enables parallelism which is essential for scaling.
The formula for self-attention at each head is as Eq.~\ref{eq:attention}, where $Q$, $k$, and $V$ are query, key, and value respectively, which all are sort of projections of the sequence. The dot product between the query and key matrices determines how much attention each token should pay to every other token, scaled by \( \sqrt{d_k} \) (the dimension of the keys) to prevent large gradients. The softmax function then normalizes these attention scores to ensure they sum to 1.
\begin{equation}
\label{eq:attention}
    \text{Attention} (Q, K, V) = \text{softmax} (\frac{QK^T}{\sqrt{d_k}}) V
\end{equation}

Multi-head attention~\autocite{vaswani2017attention} is an extension of the self-attention mechanism where the model learns multiple attention "heads". Each head learns to focus on different parts of the input sequence in parallel, allowing the model to gather a variety of representations of the same input and improving the model’s ability to capture complex relationships. These different representations are then concatenated and linearly transformed to produce the final output. 
The multi-head attention could be denoted as Eq.~\ref{eq:MultiHead_attention}, where \(W^O\) refers to the output projection weight matrix that projects the concatenated multi-head attention output back to the model's original space.
\begin{align}
\label{eq:MultiHead_attention}
    \text{MultiHead}(Q, K, V) = \text{Concat}(\text{head}_1, \text{head}_2, ..., \text{head}_h)W^O
    ,\; W^O \in \mathbb{R}^{(h \cdot d_{\text{head}}) \times d_{\text{model}}}
\end{align}

Scaling law shows the capabilities of LLMs predictably improve with model scale, so a few attention variants are proposed to reduce computation cost while sacrificing little or even no model capability. One severe memory bottleneck of scaling is the memory overhead when loading attention keys and values at every decoding step. Multi-query attention \autocite{shazeer2019fast} reduces this memory overhead by using multiple query heads but sharing a single set of key and value heads. However, multi-query attention can lead to model quality degradation. Grouped-query attention \autocite{ainslie2023gqa} uses
an intermediate (more than one, less than the number of query heads) number of key-value heads, which is shown to achieve quality close the multi-head attention while at a comparable speed to multi-query attention.


\paragraph{Tokenization} 
Tokenization transforms natural language into tokens, including characters, sub-words, words, and special tokens. For example, the sentence ``We are reviewing large language model papers'' can be transformed into a sequence of tokens like ["[CLS]", "We", "are", "review", "\#\#ing", "large", "language", "model", "papers", "[SEP]"], where "\#\#" in "\#\#ing" indicates a sub-word, and "[CLS]" and "[SEP]" are special tokens used for downstream classification tasks and indicating the end of text respectively. Tokenization brings mainly two benefits. First, the tokenization process can control the size of vocabulary, which can better suit the scaling law \autocite{kaplan2020scaling}. Besides, the combination of tokens can compose words that may be rare and even unseen in the training data.

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.7\textwidth]{Method/Figures/position_encoding.png}
% \caption{Various positional encodings are employed in LLMs. \autocite{minaee2024large}}
% \label{fig:position_encoding}
% \end{figure}

%The \textbf{position encoding} maps the word positions into informative embedding. 
\paragraph{Positional Encoding}
Since Transformer models don't have an inherent sense of position (unlike recurrent or convolutional models), the \textit{positional encoding} is used to incorporate the position information of words. Positional encoding can be categorized into \textit{absolute positional encoding} and \textit{relative positional encoding}. The absolute positional encoding uses the absolute position to calculate position embedding. For example, ~\cite{vaswani2017attention} uses the absolute positional encoding, and the corresponding positional encoding equations could be expressed as Eq.~\ref{eq:pos_en},
\begin{align}
\label{eq:pos_en}
    %PE_{pos, 2i} &= %sin(pos/10000^{2i/d_{model}})
    PE_{pos, 2i} = \sin \left(\frac{pos}{10000^{2i/d_{model}}}\right)
    \\
    %PE_{pos, 2i+1} &= %cos(pos/10000^{2i/d_{model}})
    PE_{pos, 2i+1} = \cos \left(\frac{pos}{10000^{2i/d_{model}}}\right)
\end{align}
where $pos$ is the absolute position in the sequence. $i$ is the index of the dimension of the embedding, and $d_{model}$ is the dimension of embedding that is known as the model width. These functions bring two benefits: (1) they are periodic, so nearby positions will have similar encodings, which can be useful when modeling natural language sequences. (2) using both sine and cosine ensures that the encodings for different positions are orthogonal in high-dimensional space, making it easier for the model to learn patterns.

\textcolor{purple}{[Summer: (add references here) ]}
Recently, the relative positional encoding has become more popular than absolute positional encoding because of the belief that relative position is more informative than absolute position. Instead of encoding the absolute position into a fixed embedding, relative positional encoding generates embedding based on the distance between tokens. More specifically, in attention mechanisms, the model generates "query" and "key" vectors for each token, then the model computes the interaction between a "query" token (the token currently being processed) and "key" tokens (all other tokens in the sequence).
The attention score between two tokens is computed as a dot product of their query and key vectors. Relative positional encoding modifies this by encoding how far apart the query and key tokens are.


\subsubsection{Model Architecture}
\textcolor{blue}{[YM: I have modified this part.]}
A standard Transformer would have both an encoder, for the input of texts and a decoder for the output of response. More recently, it has evolved into three main variants, each specialized for different types of language tasks: decoder-only, encoder-only, and encoder-decoder models. Table \ref{table:comparisonoftransformer} shows a comparison of three types of language tasks. These architectural variations represent different approaches to processing and generating text, each with its own strengths and primary applications. While all three variants build upon the core Transformer mechanisms, they differ in how they process context and generate outputs, leading to distinct capabilities and use cases. This section examines each of these architectural approaches and their specific characteristics.

\begin{table}[htbp]
\tiny
\centering
\label{table:comparisonoftransformer}
\begin{threeparttable}
\caption{Comparison of Transformer Architectures}
\begin{tabular}{>{\raggedright}p{2.5cm} >{\raggedright}p{3.5cm} >{\raggedright}p{3cm} >{\raggedright}p{3cm} >{\raggedright\arraybackslash}p{3.5cm}}
\toprule
\rowcolor{gray!20}
\textbf{Architecture} & \textbf{Components} & \textbf{Attention} & \textbf{Training Objective} & \textbf{Primary Use Cases} \\
\midrule
\textbf{Decoder-Only} & Stacked Decoders & Masked Self-Attention (Unidirectional) & Autoregressive Next-Token Prediction & Text Generation (e.g., GPT) \\
\textbf{Encoder-Only} & Stacked Encoders & Self-Attention (Bidirectional) & Masked Language Modeling (MLM) & Understanding Tasks (e.g., BERT) \\
\textbf{Encoder-Decoder} & Stacked Encoders \& Decoders & Self-Attention (Encoder) \& Cross-Attention (Decoder) & Sequence-to-Sequence Loss & Translation, Summarization (e.g., T5, BART) \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table}


% \begin{figure}[h]
% \centering
% \includegraphics[width=0.7\textwidth]{Method/Figures/1.png}
% \caption{An example of a transformer architecture. \autocite{vaswani2017attention}}
% \label{fig:Transformer}
% \end{figure}

\paragraph{Decoder-Only}
Decoder-only architecture refers to model structures that contain stacked layers of the decoder part of the Transformer architecture. 
Primary use cases include GPT~\autocite{radford2018improving,radford2019language,brown2020language} models and LLaMA~\autocite{touvron2023llama}. 
In this architecture, the decoder is \textit{unidirectional}, which means the input sequence is processed from left to right and the token is predicted in an \textit{autoregressive} manner, as it predicts the next token in the sequence only based on the preceding tokens. 
In this model, the primary training objective is to maximize the probability of predicting the next token conditioned on previous tokens. Trained on next-token prediction loss, decoder-only models are most suitable for generation tasks such as like text completion, story generation, and dialogue. 


\paragraph{Encoder-Only}
Encoder-only architecture, like BERT~\autocite{devlin2018bert} and RoBERTa~\autocite{liu2019roberta}, uses only the encoder part of the Transformer architecture. The key training task is \textit{Masked Language Modeling (MLM)}, where certain tokens in the input are randomly masked. During the training, the model predicts the masked tokens conditioned on other tokens from both the left and the right. Therefore, The model learns a deep \textit{bidirectional} understanding of the entire sequence by incorporating context from two directions (i.e., left and right). As a result, encoder-only models are ideal for understanding tasks, including such as text classification, question answering, and named entity recognition.


\paragraph{Encoder-Decoder}
Encoder-decoder architecture, like T5~\autocite{raffel2020exploring} and BART~\autocite{lewis2019bart}, uses both the encoder and decoder parts of the Transformer architecture. 
The encoder processes the input sequence, and the decoder generates the output sequence based on the encoded input. 
Encoder-decoder architecture tries to strike a balance between generation tasks and understanding tasks. 
Thus, it is most appropriate for sequence-to-sequence tasks such as machine translation, summarization, and text-to-text transformations.

% In the encoder-decoder architecture, the training objective is to generate a target sequence (such as a translated sentence, summary, or response) based on an input sequence (such as a source sentence or document). The loss function used for this is typically a sequence-to-sequence loss, which is based on cross-entropy loss across the entire target sequence.
% Given an input sequence \( X = (x_1, x_2, ..., x_T) \) and a target sequence \( Y = (y_1, y_2, ..., y_T) \), the model is trained to maximize the likelihood of generating the correct tokens in the target sequence, conditioned on both the input sequence and the previously generated tokens.
% For each time step \( t \), the model predicts the next token \( y_t \) based on the encoded input sequence \( X \) and the previously generated tokens \( (y_1, y_2, ..., y_{t-1}) \) in the target sequence.
% The probability of generating the next token \( y_t \) is denoted as \( p(y_t | y_1, y_2, ..., y_{t-1}, X) \).
% Finally, the sequence-to-sequence loss for a single example is the sum of the negative log probabilities (cross-entropy loss) of the true target tokens over the entire target sequence, shown in Eq.~\ref{eq:sequence_to_sequence_loss}, where \( T \) is the length of the target sequence. \( y_t \) is the true token at position \( t \) in the target sequence. \( p(y_t | y_1, y_2, ..., y_{t-1}, X) \) is the probability assigned by the model to the true token \( y_t \), given the previous tokens and the input sequence.
% \begin{align}
% \label{eq:sequence_to_sequence_loss}
%     \mathcal{L} = - \sum_{t=1}^{T} \log p(y_t | y_1, y_2, ..., y_{t-1}, X)
% \end{align}






% \textcolor{purple}{[Summer: 
% There are multiple reasons why relative positional encoding is considered more informative. 
% \begin{itemize}
%     \item \textbf{Position-invariant Relationships:} In many tasks, the relationship between words is relative, not absolute. For example, in language, the meaning of a word can depend on the word immediately before or after it, regardless of whether it appears in the middle or end of the sentence. Relative position encoding allows the model to focus on the proximity between words, which is often more critical than their absolute position.
%     \item \textbf{Better Generalization to Longer Sequences:} Relative positional encoding helps models generalize to sequences of different lengths. Since it encodes distances between tokens, rather than fixed positions, the model can handle sequences of varying lengths more effectively. Absolute positional encoding may not generalize as well to longer sequences because it doesn't take into account the relationships between words that are far apart.
%     \item \textbf{Flexibility in Capturing Local and Global Information:} Relative position encoding can capture both local (nearby tokens) and global (distant tokens) information more flexibly. In absolute positional encoding, nearby tokens have very similar encodings, but far-apart tokens have drastically different encodings. Relative encoding focuses on the distance between tokens, which allows the model to balance local context (close tokens) and global context (farther tokens).
%     \item \textbf{Efficiency in Attention Computation:} With relative positional encoding, attention scores can be directly adjusted based on the relative distance between the query and key tokens. This can improve the model's ability to focus on relevant information and ignore irrelevant tokens, making the attention computation more efficient in terms of capturing relationships in the data.
% \end{itemize}]}


\subsection{Training} %Zemian
\textcolor{blue}{[YM: If we have examples, we may borrow formatting from the following paper: Benchmarking the Capabilities of Large Language Models in Transportation System Engineering: Accuracy, Consistency, and Reasoning Behaviors. The current formatting looks informal.] [YM: the following subsections are very fragmented. If some techniques are not applied, we may remove them.]}
The training of foundation LLMs involves two key stages: (1) the pre-training phase, where the model is trained at scale on simple tasks like next-token prediction \autocite{radford2018improving} and Masked Language Modeling (MLM) \autocite{devlin2018bert}, and (2) the post-training phase, where the model is fine-tuned to follow instructions, align with human preferences, and enhance specific skills, such as coding and reasoning. When applying foundation LLMs to downstream domain-specific tasks, the performances of LLMs can be significantly improved by fine-tuning on domain-related dataset.

\subsubsection{Pre-training Phase}
Pre-training typically involves training on large, diverse text corpora (e.g., books, articles, websites) without any task-specific labels. This process is unsupervised or self-supervised, as the model learns from the structure of the data itself and captures general linguistic patterns and world knowledge. The most popular pre-training methods are next-token prediction and masked language modeling.

\paragraph{Next-token prediction} Next-token prediction, first proposed in \autocite{radford2018improving}, is a process where a language model predicts the next word or token in a sequence based on the preceding context. For example, if the input is an incomplete sentence like ``The sun is shining in the'', the model's job is to predict the most likely next word, which could be ``sky'' or ``morning,'' depending on the learned patterns from its training data. The model generates these predictions one token at a time, updating its understanding of the context as it progresses through the sequence. This approach allows the model to generate coherent and contextually appropriate text in tasks such as text completion, translation, or language generation, where each new token is predicted based on the previous ones.
As introduced in decoder-only architecture above, the objective is to minimize the autoregressive loss, shown in Eq.~\ref{eq:next_token_pred}, where \( x_1, \dots, x_T \) represent a sequence of tokens, and \( P_\theta(x_t \mid x_{1:t-1}) \) is the model’s predicted probability of the next token given the previous ones. This enables the model to learn dependencies across large text sequences, making it suitable for generative tasks like text completion and storytelling.
\begin{align}
\label{eq:next_token_pred}
     \mathcal{L}_{\text{AR}}(\theta) = -\mathbb{E}_{(x_1, \dots, x_T) \sim \mathcal{D}} \left[ \sum_{t=1}^{T} \log P_\theta(x_t \mid x_{1:t-1}) \right]
\end{align}

\paragraph{Masked language modeling} Masked Language Modeling (MLM), proposed in \autocite{devlin2018bert}, is a training approach where a model is given a sentence or sequence with some words or tokens randomly ``masked'' (hidden), and the model's task is to predict the missing tokens based on the surrounding context. For example, if the sentence is ``The cat is [MASK] on the mat,'' the model has to predict that the masked word is likely ``sitting.'' Unlike next-token prediction, MLM allows the model to learn bidirectional context, meaning it considers both the words before and after the masked token when making predictions. This method helps the model capture a deeper understanding of relationships between words and the overall sentence structure.

As introduced in encoder-only architecture above, the objective is to minimize the MLM loss, shown in Eq.~\ref{eq:mlm_in_training}, where \( M \) represents the set of masked tokens, and \( x_{\backslash t} \) denotes the sequence with the masked tokens excluded. By doing this, the model captures bidirectional context and learns relationships between words in a sentence, leading to strong performance on understanding tasks like classification, question answering, and sentence encoding.
\begin{align}
\label{eq:mlm_in_training}
         \mathcal{L}_{\text{MLM}}(\theta) = -\mathbb{E}_{(x_1, \dots, x_T) \sim \mathcal{D}} \left[ \sum_{t \in M} \log P_\theta(x_t \mid x_{\backslash t}) \right]
\end{align}

Throughout pre-training, models typically optimize these objectives over vast corpora to develop a generalized understanding of language. This process results in learning a set of parameters \( \theta \) that capture statistical properties of text and linguistic patterns, without being specialized for specific downstream tasks.


\subsubsection{Post-training Phase}
In post-training stage, the pre-trained model is further trained to follow instructions, align with human preferences, and adapt to specific tasks. The optimization objective can vary depending on the purpose.

\paragraph{Instruction tuning} Instruction tuning is the process of supervised fine-tuning large language models on instruction datasets to better understand and follow natural language instructions. For example, in instruction tuning, the model might be given tasks like “Summarize this paragraph,” “Translate this sentence into Spanish,” or “Explain the steps to solve this math problem.” By exposing the model to a wide range of task-specific instructions during training, the model learns how to generalize across various types of commands, making it more flexible and capable of handling diverse user requests. This approach improves the model’s ability to perform tasks directly from natural language instructions without needing task-specific fine-tuning each time.

Models are fine-tuned on datasets where the objective is to maximize the likelihood of generating correct responses to specific instructions. For this, the fine-tuning loss is similar to next-token prediction but adapted for task-oriented interactions:
\begin{align}
    \mathcal{L}_{\text{FT}}(\theta) = -\mathbb{E}_{(x_1, \dots, x_T) \sim \mathcal{D}_{\text{task}}} \left[ \sum_{t=1}^{T} \log P_\theta(x_t \mid x_{1:t-1}) \right]
\end{align}
 where \( \mathcal{D}_{\text{task}} \) represents the task-specific data. This allows the model to become proficient at generating task-appropriate and user-aligned outputs.

\paragraph{Alignment with human preferences} 
Alignment with human preferences refers to the process of adjusting LLM behavior to ensure it generates outputs that are more aligned with human values, judgments, and expectations. The model is trained using human evaluations to refine its outputs. For example, the model might generate several responses to a query, and human evaluators rank those responses based on their quality, usefulness, or safety. The model then learns from this feedback to prioritize responses that humans prefer. This process helps ensure that the model produces helpful, coherent, and less harmful outputs, mitigating issues like biased, inappropriate, or dangerous responses. The goal is to make AI more user-friendly, ethical, and safe for practical applications. 

The most popular method for aligning models with human preferences is Reinforcement Learning from Human Feedback (RLHF) \autocite{ouyang2022training, lightman2023let}, where human evaluators provide feedback on model outputs, and then a reward model is trained on human preference data to predict human scores on model outputs. Then, LLM is fine-tuned using reinforcement learning with rewards from the reward model. Alternatively, one can bypass the usage of reward models and reinforcement learning by using a direct loss function on preference data (e.g., direct preference optimization (DPO) \autocite{rafailov2024direct}).

% More Specifically, during the RLHF process, a reward model \( R(x) \) is trained to score outputs, and the LLM is fine-tuned using a policy gradient method to maximize the expected reward, shown in Eq.~\ref{eq:reward_model}. This helps adjust the model's responses to ensure they are aligned with human expectations and ethical standards.

% \begin{align}
% \label{eq:reward_model}
%          \mathcal{L}_{\text{RLHF}}(\theta) = -\mathbb{E}_{x \sim P_\theta} \left[ R(x) \right]
% \end{align}



More specifically, to refine the LLM's outputs based on human preferences, a reward model \(R_\phi(x)\) is trained using human feedback on the outputs generated by the LLM. This feedback is typically gathered through a process of ranking or scoring. Given a set of prompts, the LLM generates multiple responses. Human annotators are asked to rank these responses based on various criteria such as accuracy, coherence, helpfulness, and safety. For example, if given two responses \(x_1\) and \(x_2\), the annotators might prefer \(x_1\) over \(x_2\), providing a ranking \(x_1 \succ x_2\).
The reward model \(R_\phi(x)\) is trained to predict the human preference rankings. It assigns a scalar reward score to each model-generated response based on how well it aligns with the human-provided rankings. The objective function for the reward model is formulated as a pairwise ranking loss, shown in Eq.~\ref{eq:reward_loss}, where \(x_1 \succ x_2\) indicates that human annotators preferred \(x_1\) over \(x_2\), and \(\mathcal{D}_{\text{human}}\) is the dataset of human feedback. The model \(R_\phi(x)\) learns to predict higher rewards for responses that align more closely with human preferences.
\begin{align}
\label{eq:reward_loss}
      \mathcal{L}_{\text{reward}}(\phi) = -\mathbb{E}_{(x_1, x_2) \sim \mathcal{D}_{\text{human}}} \left[ \log \frac{e^{R_\phi(x_1)}}{e^{R_\phi(x_1)} + e^{R_\phi(x_2)}} \right]
\end{align}

  



Once the reward model is trained, it is used to guide the LLM through reinforcement learning (RL). The goal is to fine-tune the LLM so that its outputs maximize the reward function learned from human feedback.
The LLM can be considered a policy \( \pi_\theta(x \mid z) \), parameterized by \(\theta\), where \(z\) is a given input (e.g., a prompt), and \(x\) is the model’s output (e.g., a response). The objective of reinforcement learning is to find the optimal parameters \(\theta^*\) that maximize the expected reward, shown in Eq.~\ref{eq:maximize_the_expected_reward}, where \(R_\phi(x)\) is the reward score provided by the reward model.
\begin{align}
\label{eq:maximize_the_expected_reward}
      \theta^* = \arg\max_\theta \mathbb{E}_{x \sim \pi_\theta(x \mid z)} \left[ R_\phi(x) \right]
\end{align}

A popular RL algorithm used for fine-tuning LLMs is Proximal Policy Optimization (PPO). PPO is chosen due to its stability and efficiency in handling large-scale models. The PPO objective can be written as Eq.~\ref{eq:ppo}, where \(r(\theta)\), shown in Eq.~\ref{eq:probability_ratio_between_policies}, is the probability ratio between the current policy and the previous policy and \(\epsilon\) is a hyperparameter that controls the clipping range. The clipping prevents large updates, ensuring stable training and avoiding policy collapse. By maximizing this objective, the model learns to generate outputs that are more aligned with human feedback.
\begin{align}
\label{eq:ppo}
      \mathcal{L}_{\text{PPO}}(\theta) = \mathbb{E}_{x \sim \pi_\theta} \left[ \min\left( r(\theta), \text{clip}(r(\theta), 1 - \epsilon, 1 + \epsilon) \right) \cdot R_\phi(x) \right]
\end{align}
\begin{align}
\label{eq:probability_ratio_between_policies}
  r(\theta) = \frac{\pi_\theta(x \mid z)}{\pi_{\theta_{\text{old}}}(x \mid z)}
\end{align}

To further improve the model’s alignment over time, the RLHF process can involve iterative feedback loops. In each loop: New prompts are generated, and model responses are evaluated by human annotators. The reward model is updated with additional feedback, improving its ability to reflect human preferences. The LLM is fine-tuned again using updated reinforcement learning objectives, enhancing the quality of generated outputs.
This iterative process ensures that the model continually improves in terms of ethical alignment, user-friendliness, and the ability to produce safe, high-quality content. Over successive cycles, models trained with RLHF have demonstrated remarkable improvements in performing nuanced tasks, maintaining factual accuracy, and adhering to ethical standards in response generation.



In summary, the overall objective of RLHF is to maximize the reward function \(R_\phi(x)\) derived from human feedback, which can be written as:
\[
\mathcal{L}_{\text{RLHF}}(\theta) = -\mathbb{E}_{x \sim \pi_\theta(x \mid z)} \left[ R_\phi(x) \right]
\]
with the policy \(\pi_\theta(x \mid z)\) being optimized using PPO or a similar reinforcement learning algorithm to ensure stability and gradual policy improvement.

% Benefits of RLHF
% - Safety and ethical alignment: RLHF allows models to be fine-tuned to avoid producing harmful, biased, or unethical content. By incorporating human judgment into the reward function, LLMs become more attuned to societal norms and values.
% - Customization to user preferences: Fine-tuning via RLHF enables models to generate responses that are more helpful, concise, and aligned with user-specific needs, improving user satisfaction.
% - Task-specific performance: RLHF can also enhance performance on specific tasks (e.g., dialogue systems, question-answering) by integrating human feedback on task quality, leading to more accurate and contextually relevant outputs.


\paragraph{Fine-tuning for downstream tasks} 
When applying foundation LLMs to downstream tasks, it is desirable to fine-tune LLMs to develop specialized capabilities, such as code generation or mathematical reasoning. For instance, models designed for code generation (e.g., Codex) are fine-tuned on programming languages, optimizing for accuracy in predicting code tokens, based on an objective similar to the next-token prediction but adapted for code, as shown in Eq.~\ref{eq:fine_tune_code}, where \( c_1, \dots, c_T \) represent a sequence of code tokens, and \( \mathcal{D}_{\text{code}} \) is the dataset containing programming code.
\begin{align}
\label{eq:fine_tune_code}
         \mathcal{L}_{\text{code}}(\theta) = -\mathbb{E}_{(c_1, \dots, c_T) \sim \mathcal{D}_{\text{code}}} \left[ \sum_{t=1}^{T} \log P_\theta(c_t \mid c_{1:t-1}) \right]
\end{align}  

When applying foundation LLMs to domain-specific tasks (e.g., legal text analysis, medical diagnosis), the model's performance can be significantly improved by fine-tuning on domain-specific datasets. The loss function used during domain-specific fine-tuning is similar to the original objective but applied to data from the desired field, as shown in Eq.~\ref{eq:domain_specific_fine_tune}, where \( \mathcal{D}_{\text{domain}} \) represents a dataset from the specific domain. This fine-tuning ensures that the model can handle domain-specific vocabulary, concepts, and tasks with greater accuracy and relevance.
\begin{align}
\label{eq:domain_specific_fine_tune}
    \mathcal{L}_{\text{domain}}(\theta) = -\mathbb{E}_{(x_1, \dots, x_T) \sim \mathcal{D}_{\text{domain}}} \left[ \sum_{t=1}^{T} \log P_\theta(x_t \mid x_{1:t-1}) \right]
\end{align}

Fine-tuning algorithms include traditional approaches like fully fine-tuning and more recent techniques designed to optimize memory and computational resources, such as adapter-based fine-tuning and parameter-efficient fine-tuning (PEFT).

Fully fine-tuning is the conventional approach where all the parameters of the pre-trained model are updated during the fine-tuning process. This method provides the most flexibility, allowing the model to fully adjust to the target task. However, it comes at the cost of high computational and memory overhead, especially for very large models. Fully fine-tuning is typically used when there is ample task-specific data and computational resources. Despite its effectiveness, this approach can be inefficient for smaller datasets or cases where the model must adapt to multiple tasks, each requiring separate fine-tuning.

To address these issues, adapter-based fine-tuning has gained popularity as a more efficient alternative \autocite{houlsby2019parameter}. In this method, small adapter modules are introduced between the layers of the pre-trained model, and only these adapters are fine-tuned while the rest of the model remains frozen. This dramatically reduces the number of parameters that need updating, leading to significant savings in both memory and computation. Adapter-based methods are particularly advantageous in multi-task learning scenarios, where different adapters can be trained for different tasks without retraining the entire model. This approach also allows for modular adaptation, making it possible to switch between different tasks by simply replacing the adapter layers.

Another increasingly popular approach is parameter-efficient fine-tuning (PEFT), which focuses on reducing the number of parameters updated during fine-tuning. Methods like Low-Rank Adaptation (LoRA) add low-rank modifications to the model’s parameters, allowing for efficient fine-tuning with fewer updates \autocite{hu2021lora}. By reducing the complexity of fine-tuning, PEFT methods make it feasible to fine-tune large models with fewer resources, offering an attractive solution for resource-constrained environments. Additionally, prompt-based fine-tuning, such as prefix tuning \autocite{li2021prefix}, has emerged as a highly efficient method. Instead of altering model parameters, this technique guides the model’s behavior through carefully designed input prompts or task-specific prefixes, making the model adaptable to different tasks with minimal changes to the model.


\subsection{Prompt Engineering} %Ziyan
Prompt engineering is the process of crafting the optimal input for LLMs to achieve the best performance. As an emerging field, the practice of prompt engineering varies significantly depending on the application domain. However, several notable works have proposed promising approaches that are now widely adopted. The most basic form of a prompt is simply a description of the task, commonly referred to as zero-shot prompting. For example, \textit{Prompt}: ``Is the following statement true or false: `The first woman to win an Olympic gold medal was Countess Hélène de Pourtalès.' '' \textit{Output}: ``True.'' In this case, no additional context is provided to the LLM; the prompt simply presents the question that needs to be answered. As a result, the LLM relies on its pre-existing knowledge of sports history to generate the output. For straightforward tasks like this, zero-shot prompting can be sufficient. However, for more complex tasks, such as logical reasoning, zero-shot prompts are often less effective.
Typically, a more advanced prompt includes a description of the task, the LLM's role, a specific question, examples, and relevant context. In addition to designing the content of the prompt, the structure of the prompt can vary, with techniques such as few-shot prompting, chain-of-thought~\autocite{wei2022chain}, tree-of-thought~\autocite{yao2024tree}, and graph-of-thought~\autocite{besta2024graph}, among others. 

\subsubsection{In-Context Learning}
The goal of In-Context Learning (ICL) is to provide context to LLMs in the form of demonstrations~\autocite{dong2024surveyincontextlearning}. ICL is typically performed on pre-trained LLMs and does not require direct parameter updates to the models. The selection of demonstrations and instructions is crucial to the performance of ICL. As a result, various follow-up works have been proposed to enhance ICL capabilities, focusing on aspects such as demonstration selection and organization~\autocite{qin2023context,he2023icl}, and reformatting, using a range of machine learning and optimization techniques~\autocite{dong2022survey}.

\subsubsection{Few-Shot Prompting}
Slightly more complicated than zero-shot prompts, a few-shot prompt consists of a few input-output example pairs, which help LLMs understand the task through repetition, pattern recognition and generalization. This prompting method is particularly useful when the correct answer can be inferred from similar tasks. For example, few-shot prompts can be employed for text classification tasks, as evaluated in ~\autocite{liu2023pre}. In single-sentence classification tasks, several examples of input text (e.g., ``One of the other reviewers has mentioned that after watching just 1 Oz episode, you'll be hooked.''), available options (e.g., ``Is it great or terrible?''), and output (e.g., ``It is great.'') help the model learn the classification pattern. However,~\cite{lu2021fantastically} suggests that LLMs are sensitive to the order of examples provided in few-shot prompting. Therefore, various permutations of few-shot prompts should be tested to identify the most effective order.

\subsubsection{Chain-of-Thought Prompting}
A limitation of few-shot prompting is that LLMs can sometimes generate the correct answer by chance, especially when there are only a few possible options. However, this approach may fail to help the LLM grasp the underlying logic of the task, which becomes a significant issue when solving problems that require complex reasoning.
Chain-of-thought prompting~\autocite{wei2022chain} improves the performance of LLMs on complex tasks, particularly those requiring mathematical reasoning and arithmetic calculations. Moreover, chain-of-thought prompts have been shown to be effective for decision-making tasks, such as dynamic programming~\autocite{feng2024towards}. This can be achieved either by adding direct phrases like ``think step by step'' to the prompt or by including triples of $\langle$input, chain-of-thought, output$\rangle$ for solving the task step-by-step. For example: Bill has 5 apples. He buys 2 more buckets of apples from the market, with each bucket containing 6 apples. How many apples does Bill have now? Chain-of-thought: Bill starts with 5 apples and buys 2 buckets, each containing 6 apples. So, the total number of apples is $5 + 2 \times 6 = 17$. Output: The answer is 17.

\subsubsection{CoT Prompting with Self-Consistency}
Also known as the multiple chain-of-thought prompting technique,~\cite{wang2022self} introduces a ``sample-and-marginalize'' procedure to identify the most consistent answer for complex tasks requiring deliberate reasoning. Specifically, LLMs generate a diverse set of possible reasoning paths using chain-of-thought prompting and then reach a consensus through majority voting.
However, it is important to note that this technique is most effective for tasks with a fixed set of correct answers, as it relies on self-consistency. Open-ended tasks, on the other hand, require a more careful design of consistency metrics to achieve reliable outcomes.

\subsubsection{Tree-of-Thought Prompting}
More advanced than chain-of-thought prompting with self-consistency, the tree-of-thought~\autocite{yao2024tree} technique considers multiple potential reasoning paths, allowing for self-evaluation, backtracking, and looking ahead. It can be seen as a generalization of chain-of-thought. Intuitively, the reasoning paths branch out like a tree, with unpromising branches being pruned. Each reasoning step acts as an intermediate stop, helping to decompose complex tasks. For instance, when solving a multi-step problem like the game of 24, tree-of-thought first breaks down the task into intermediate steps. From each current node, tree-of-thought generates samples of potential thoughts and expands them into subsequent steps. A heuristic is then used to evaluate the branches. Since the structure is tree-like, search algorithms such as breadth-first search and depth-first search can be applied to guide the tree-of-thought process.

\subsubsection{Graph-of-Thought Prompting}
\textcolor{blue}{[ym: may add a graph for this]}
Performing even better on tasks like sorting, keyword counting, and document merging, the graph-of-thought~\autocite{besta2024graph} prompting technique allows intermediate reasoning steps generated by LLMs to first expand and then connect with each other, forming a large network of thoughts. The key innovation in graph-of-thought is the aggregation process, where edges from separate reasoning paths converge at a shared vertex. This merging process requires sorting and ranking actions to organize different branches into the correct order selectively. Graph-of-thought prompting also holds potential for sequential planning tasks, where multiple goals exist and must be completed in a specific order.

\subsubsection{Automated Prompt Engineer}
Aside from the manual prompt engineering methods mentioned earlier, some works have proposed approaches for generating automated prompts. In tasks such as retrieval and reasoning, Automated Prompt Engineering (APE) has been shown to outperform state-of-the-art manual prompts (e.g., ``let's think step by step'') (e.g.,~\cite{jin2024apeer,sahoo2024systematic}), while significantly reducing the need for human trial-and-error efforts. Introduced by~\cite{zhou2022large}, APE leverages LLMs to search over a set of generated candidate prompts. Framed as a black-box optimization problem, each candidate prompt is assigned a score, and Monte Carlo search methods are employed to iteratively refine and improve the best-performing candidate prompts.


\subsection{Retrieval-Augmented Generation}
%Ziyan 
\textcolor{blue}{[YM: need a connection between two sections]}The primary goal of Retrieval-Augmented Generation (RAG) is to enhance the factual accuracy of large language models (LLMs) and reduce the likelihood of hallucinations~\autocite{lewis2020retrieval}. For tasks that require specific domain knowledge or information not included in their training corpus, RAG serves as an effective solution by enabling the model to retrieve relevant information before generating text. As the name implies, RAG consists of two key components: the retriever and the generator. The retriever’s role is to fetch relevant information from an external knowledge source, while the generator uses both the original prompt and the retrieved context to produce a more informed response.
A common implementation of RAG involves segmenting the external knowledge base into smaller chunks, which are then encoded into vector representations using a pre-trained embedding model. Similarly, the prompt is encoded as a vector, and the similarity between the prompt vector and each chunk in the database (often measured by cosine similarity) is computed. The top-ranked chunks, representing the most relevant information, are then passed to the generation phase. In this phase, the original prompt and the retrieved context are combined into a comprehensive input, enabling the LLM to produce more accurate, contextually enriched answers.
Recent works have introduced advanced variations of RAG, such as Advanced RAG and Modular RAG~\autocite{gao2023retrieval}. Advanced RAG enhances the retrieval process by incorporating optimization techniques that improve either the pre-retrieval phase, the post-retrieval phase, or both. On the other hand, Modular RAG is a more complex framework that introduces additional components beyond the basic retriever and generator. For instance, ~\cite{wang2023knowledgpt} integrates a search module to bridge the gap between LLMs and multiple sources of knowledge, allowing the model to pull information from various databases, improving accuracy and up-to-date information. 

\subsection{Evaluation Metrics of LLMs}  % zemian
\subsubsection{General metrics}
LLMs are evaluated using a variety of standard, general-purpose metrics that apply across a wide range of natural language processing tasks. These metrics focus on assessing the performance of models in terms of accuracy, fairness, robustness, and calibration.

\textbf{Accuracy.} This is one of the most fundamental metrics used to assess how well a model's outputs match the ground truth or expected outcomes. Specific accuracy-related metrics include:
    \begin{itemize}
        \item \textit{Exact Match}: This measures whether the generated text exactly matches the reference answer.
        \item \textit{F1 Score}: A metric that combines precision and recall to provide a harmonic mean, commonly used in classification tasks.
        \item \textit{ROUGE Score}: Used primarily for evaluating tasks like text summarization and machine translation by measuring overlap between the generated and reference texts.
    \end{itemize}
    
\textbf{Calibration.} Calibration evaluates the alignment between the model's confidence in its predictions and the actual likelihood of those predictions being correct. Metrics here include:
    \begin{itemize}
        \item \textit{Expected Calibration Error} \autocite{pmlr-v70-guo17a}: Measures the difference between confidence levels and accuracy.
        \item \textit{Area Under the Curve (AUC)}: This is often used to measure model performance in terms of coverage and accuracy in selective prediction settings.
    \end{itemize}
    
\textbf{Fairness.} Fairness metrics aim to measure whether a model treats different demographic groups equally. These include:
    \begin{itemize}
        \item \textit{Demographic Parity Difference}: Evaluates the difference in treatment across groups in terms of positive outcomes.
        \item \textit{Equalized Odds Difference}: Measures whether the model produces similar outcomes across groups, controlling for actual outcomes.
    \end{itemize}
    
\textbf{Robustness.} Robustness evaluates the model's resilience to changes or attacks in the input. Common robustness metrics include:
    \begin{itemize}
        \item \textit{Attack Success Rate} \autocite{wang2021adversarial}: Measures the model’s vulnerability to adversarial attacks.
        \item \textit{Performance Drop Rate} \autocite{zhu2023promptbench}: Quantifies the performance degradation after adversarial modifications to the prompts.
    \end{itemize}

\subsubsection{Metrics for specific tasks}
In addition to general evaluation metrics, many customized metrics are developed to assess LLMs in specific domains or tasks. These metrics are tailored to the unique demands of particular applications and are used to evaluate capabilities that general metrics might not adequately capture.


\textbf{Multimodal Task Benchmarks.} For evaluating the performance of \textit{Multimodal Large Language Models (MLLMs)}, benchmarks like \textit{MMBench} \autocite{liu2023mmbench} focus on assessing vision-language models by evaluating the model's capability to process and understand both visual and textual data. This includes performance across tasks such as perception and cognition.
    
\textbf{Reasoning Tasks.} The \textit{Advanced Reasoning Benchmark} \autocite{sawada2023arb} focuses on evaluating LLMs in complex reasoning tasks across multiple domains, pushing models to handle more sophisticated problem-solving. More recently, a few evaluation methods have been proposed to evaluate specific reasoning tasks, such as coding (e.g., SWE bench \autocite{jimenez2024swebench}) and machine learning engineering \autocite{chan2024mlebenchevaluatingmachinelearning}.

\textbf{Ethics and Bias in LLMs.} \textit{TRUSTGPT} is a customized benchmark designed to test the ethical considerations of LLMs, including metrics related to \textit{toxicity}, \textit{bias}, and \textit{value alignment} \autocite{huang2023trustgpt}.

\subsection{Comparison of main-stream LLM Models}
%(GPT-3, GPT-4, GPT-4o, Mistral, Vicuna-13B, Falcon, Davinci, Claude-V1, Alpaca-13B)

LLMs are transformer-based pre-trained models (PLMs) with tens to hundreds of billions of parameters, demonstrating superior language understanding, generation, and emergent capabilities compared to smaller models. Notable LLM families include GPT, LLaMA, and PaLM~\autocite{zhao2023survey,minaee2024large}.

\subsubsection{GPT Family}

Developed by OpenAI, it includes models like GPT-3, GPT-4, CODEX, and ChatGPT. 
\begin{itemize}
    \item \textbf{GPT-3}~\autocite{brown2020language} is an autoregressive model with 175 billion parameters, showcasing emergent abilities like in-context learning and excelling in various NLP tasks.
    \item \textbf{CODEX}~\autocite{chen2021evaluating} is fine-tuned for programming, powering GitHub Copilot.
    \item \textbf{WebGPT}~\autocite{nakano2021webgpt} uses a web browser for answering open-ended questions, trained through reinforcement learning.
    \item \textbf{InstructGPT}~\autocite{ouyang2022training} was trained with human feedback to align with user intent, leading to improved truthfulness.
    \item \textbf{ChatGPT}~\footnote{\hyperlink{https: //openai.com/blog/chatgpt}{https: //openai.com/blog/chatgpt}}, based on GPT-3.5 and later GPT-4, is widely used for dialogue tasks.
    \item \textbf{GPT-4}~\autocite{achiam2023gpt} is a multimodal model that takes both text and image inputs, demonstrating strong performance in professional exams.
\end{itemize}


\subsubsection{LLaMA Family}
Released by Meta, LLaMA models are open-source, making them popular for research and task-specific applications.
\begin{itemize}
    \item \textbf{LLaMA}~\autocite{touvron2023llama} models range from 7B to 65B parameters and are based on GPT-3's architecture with modifications like SwiGLU activation.
    \item \textbf{LLaMA-2}~\autocite{touvron2023llama} includes Chat models fine-tuned for dialogue and developed in partnership with Microsoft.
    \item \textbf{Alpaca}~\autocite{taori2023alpaca}, \textbf{Vicuna}~\footnote{\hyperlink{https://lmsys.org/blog/2023-03-30-vicuna/}{https://lmsys.org/blog/2023-03-30-vicuna/}}, and \textbf{Guanaco}~\footnote{\hyperlink{https://guanaco-model.github.io/}{https://guanaco-model.github.io/}} are models fine-tuned from LLaMA for specific tasks, with efficient fine-tuning techniques like \textbf{QLoRA}~\autocite{dettmers2024qlora}.
    \item \textbf{Mistral-7B}~\autocite{jiang2023mistral} is a smaller but high-performing model outperforming other open-source models like LLaMA-2-13B.
\end{itemize}

\subsubsection{PaLM Family}

Developed by Google, PaLM models excel in large-scale learning tasks.
\begin{itemize}
    \item \textbf{PaLM}~\autocite{chowdhery2023palm} is a 540B parameter model, achieving state-of-the-art few-shot learning results.
    \item \textbf{Flan-PaLM}~\autocite{chung2024scaling} is fine-tuned with chain-of-thought data, outperforming previous models.
    \item \textbf{PaLM-2}~\autocite{anil2023palm} improves upon PaLM, offering better multilingual and reasoning capabilities.
    \item \textbf{Med-PaLM}~\autocite{singhal2023large} and \textbf{Med-PaLM 2}~\autocite{singhal2023towards} are domain-specific versions for medical question answering.
\end{itemize}


\subsubsection{Other LLMs}
\textcolor{blue}{[ym: may not need all of them]}
\begin{itemize}
    \item \textbf{FLAN}~\autocite{wei2021finetuned}: Instruction-tuned model improving zero-shot performance.
    % \item \textbf{Gopher}~\autocite{rae2021scaling}: A 280B parameter model with state-of-the-art performance across diverse tasks.
    \item \textbf{T0}~\autocite{sanh2021multitask}: Designed for mapping natural language tasks into a prompted form.
    % \item \textbf{ERNIE 3.0}~\autocite{sun2021ernie}: Knowledge-enhanced model for NLP tasks.
    % \item \textbf{RETRO}~\autocite{borgeaud2022improving}: Enhanced by conditioning on retrieved document chunks.
    % \item \textbf{GLaM}~\autocite{du2022glam}: Uses a mixture-of-experts architecture for efficient scaling.
    % \item \textbf{LaMDA}~\autocite{thoppilan2022lamda}: Specialized for dialogue and pretrained on public web text.
    % \item \textbf{OPT}~\autocite{zhang2022opt}: Open pre-trained transformers ranging up to 175B parameters.
    % \item \textbf{Chinchilla}~\autocite{hoffmann2022training}: Compute-optimal training with improved efficiency.
    % \item \textbf{Galactica}~\autocite{taylor2022galactica}: Focused on reasoning about scientific knowledge.
    \item \textbf{CodeGen}~\autocite{nijkamp2022codegen}: Open-sourced model for programming languages.
    % \item \textbf{AlexaTM}~\autocite{soltan2022alexatm}: Multilingual seq2seq model excelling in few-shot learning.
    % \item \textbf{Sparrow}~\autocite{glaese2022improving}: Trained for safe and factual information-seeking dialogues.
    \item \textbf{Minerva}~\autocite{lewkowycz2022solving}: Handles quantitative reasoning for mathematics and science.
    % \item \textbf{MoD (UL2)}~\autocite{tay2022ul2}: Generalizes various self-supervision paradigms in NLP.
    \item \textbf{BLOOM}~\autocite{le2023bloom}: A 176B-parameter open-access model trained on 59 languages.
    % \item \textbf{GLM}~\autocite{zeng2022glm}: Bilingual model open-sourced to compete with GPT-3.
    % \item \textbf{Pythia}~\autocite{biderman2023pythia}: Suite of models trained on public data for research study.
    % \item \textbf{Orca}~\autocite{mukherjee2023orca}: Learns from large foundation models like GPT-4.
    % \item \textbf{StarCoder}~\autocite{li2023starcoder}: Specializes in programming language tasks with competitive performance.
    % \item \textbf{KOSMOS-1}~\autocite{huang2023language}: Multimodal model trained on text and image data.
    \item \textbf{Gemini}~\autocite{team2023gemini}: Supports multiple modalities including image, audio, and text.
\end{itemize}

Additionally, frameworks and techniques like InnerMonologue~\autocite{huang2022inner}, Megatron-Turing NLG~\autocite{smith2022using}, LongFormer~\autocite{beltagy2020longformer}, OPT-IML~\autocite{iyer2022opt}, MeTaLM~\autocite{hao2022language}, Dromedary~\autocite{sun2024principle}, Palmyra~\footnote{\hyperlink{https://dev.writer.com}{https://dev.writer.com}}, Camel~\footnote{\hyperlink{https://dev.writer.com}{https://dev.writer.com}}, Yalm~\footnote{\hyperlink{https://github.com/yandex/YaLM-100B}{https://github.com/yandex/YaLM-100B}}, MPT~\autocite{mosaicml2023introducing}, ORCA 2~\autocite{mitra2023orca}, Gorilla~\autocite{patil2023gorilla}, PAL~\autocite{gao2023pal}, Claude~\footnote{\hyperlink{https://www.anthropic.com/news/introducing-claude}{https://www.anthropic.com/news/introducing-claude}}, CodeGen2~\autocite{nijkamp2023codegen2}, Zephyr~\autocite{tunstall2023zephyr}, Grok~\footnote{\hyperlink{https://grok.x.ai/}{https://grok.x.ai/}}, Qwen~\autocite{bai2023qwen}, Mamba~\autocite{gu2023mamba}, Mixtral-8x7B~\footnote{\hyperlink{https://mistral.ai/news/mixtral-of-experts/}{https://mistral.ai/news/mixtral-of-experts/}}, DocLLM~\autocite{wang2023docllm}, DeepSeek-Coder~\autocite{guo2024deepseek}, FuseLLM-7B~\autocite{wan2024knowledge}, TinyLlama-1.1B~\autocite{zhang2024tinyllama}, and LLaMA-Pro-8B~\autocite{wu2024llama} have also contributed to LLM advancements.





%\subsection{Techniques of LLM for transportations}

%Downstream tasks

%\subsubsection{How LLMs are built}

\subsection{Data} %summer
With the emergence of ChatGPT\footnote{\hyperlink{https://openai.com/index/chatgpt/}{https://openai.com/index/chatgpt/}} in November 2022, which demonstrated strong performance in general-purpose language understanding and generation, LLMs have garnered significant attention from industry, academia, and the general public.
The extraordinary language understanding and generation capabilities of LLMs like ChatGPT are fundamentally attributed not only to the scale of the models, the number of parameters, and the training paradigms but, more importantly, to the fact that they are trained on massive amounts of text data. 
% As the saying goes, “You can’t make a silk purse out of a sow’s ear.” 
Without high-quality datasets as the foundation, it is challenging to cultivate the flourishing branches and leaves of LLMs. Therefore, the construction and analysis of LLM datasets is a field deserving of attention~\autocite{liu2024datasets}.

The datasets emerging due to the rise of LLMs undoubtedly also reflect the characteristics of traditional NLP datasets. However, unlike the task-centric construction of the latter, such as datasets for question answering, text translation, text summarization, named entity recognition, etc., LLMs have driven a shift toward construction that centers around ``tasks and stages'' in dataset development. LLM datasets are not only categorized based on tasks but also aligned with different stages of LLM development. From the initial pre-training stage to the final evaluation stage, LLM datasets can be categorized into four types: (1) pre-training corpora, (2) instruction fine-tuning datasets, (3) preference datasets, and (4) evaluation datasets. 

\subsubsection{Pre-training Corpora}
Pre-training corpora are extensive collections of text data that serve as the foundation for LLMs during the pre-training phase. These corpora, which are the largest among all types of datasets, encompass diverse text types, including webpages, academic materials, and books, as well as domain-specific data such as legal documents and medical textbooks. Pre-training corpora can be categorized into \textit{general corpora}, which provide broad language knowledge from mixed domains, and \textit{domain-specific corpora}, \textcolor{blue}{[YM: in APA style, we generally use italics for emphasis, not bold characters]} which focus on specialized knowledge for particular fields. These corpora enable LLMs to learn grammar, semantics, and contextual information, enhancing their general language understanding, generalization abilities, and performance on downstream tasks. Additionally, by incorporating texts in multiple languages, pre-training corpora support multilingual processing and cross-lingual tasks, making them crucial for the development and future potential of LLMs.

\paragraph{General pre-training corpora} 
General pre-training corpora benefit from their inclusion of text content that is not confined to a single domain, making them more suitable for training general foundational models. The data types of general pre-training corpora can be classified into eight major categories: webpages, language texts, books, academic materials, code, parallel corpora, social media, and encyclopedias.
\begin{itemize}
    \item \textbf{Webpages} are the most common type of data in general pre-training corpora, consisting of text collected by crawling the internet and characterized by their massive scale, dynamic updates, multilingual content, rich themes, and semi-structured HTML format.~\autocite{xue2020mt5,penedo2023refinedweb,raffel2020exploring,abadji2022towards,yuan2021wudaocorpora} 
    % However, it is important to note that such massive web content is often not clean and contains a lot of irrelevant information, such as advertisements, navigation bars, and more. Additionally, there is the presence of pornographic content, violence, machine-generated spam, and sensitive information involving personal privacy, necessitating extensive cleaning processes to remove noise, privacy-related, and irrelevant information. \textbf{Two primary methods are used to construct webpage corpora}: (1) \textbf{refining and cleaning data from Common Crawl}, as seen in datasets like RefinedWeb~\autocite{penedo2023refinedweb}, C4~\autocite{raffel2020exploring}, mC4~\autocite{xue2020mt5}, and OSCAR~\autocite{abadji2022towards}; and (2) \textbf{independently crawling raw webpages and applying cleaning processes}, as done in WuDaoCorpora-Text~\autocite{yuan2021wudaocorpora} and other multi-category corpora~\autocite{he2023wanjuan,chen2023tigerbot}, to create high-quality multilingual datasets for LLM pre-training.
    % \item \textbf{Daily Language Texts} consist of two main types: \textit{electronic text data constructed from diverse written and spoken language resources}, such as the American National Corpus (ANC)~\footnote{\hyperlink{https://anc.org/}{https://anc.org/}} and British National Corpus (BNC)~\footnote{\hyperlink{http://www.natcorp.ox.ac.uk/}{http://www.natcorp.ox.ac.uk/}}, which contain 22 million and 100 million words respectively; and \textit{electronic text data constructed based on relevant written materials in various fields or topics}, such as FinGLM~\footnote{\hyperlink{https://github.com/MetaGLM/FinGLM}{https://github.com/MetaGLM/FinGLM}} for financial reports, TigerBot-law~\autocite{chen2023tigerbot} for legal regulations, and News-crawl~\footnote{\hyperlink{https://data.statmt.org/news-crawl/}{https://data.statmt.org/news-crawl/}} for multilingual news articles from 59 languages.
    % \item \textbf{Books} data is characterized by longer text, higher quality, and a broad range of subjects, which enhances LLMs' ability to learn deep language features, context, and cultural nuances~\autocite{zhu2015aligning,rae2019compressive,bandy2021addressing}. 
    % Sources like Smashwords~\footnote{\hyperlink{https://www.smashwords.com/}{https://www.smashwords.com/}}, Project Gutenberg~\footnote{\hyperlink{https://www.gutenberg.org/}{https://www.gutenberg.org/}}, Toronto Book Corpus~\autocite{zhu2015aligning}, PG-19~\autocite{rae2019compressive}, BookCorpusOpen~\autocite{bandy2021addressing} and Anna's Archive~\footnote{\hyperlink{https://annas-archive.org/datasets}{https://annas-archive.org/datasets}} provide extensive book data, enabling the creation of large-scale, diverse, and domain-specific book corpora that can improve the performance and adaptability of language models.
    % \item \textbf{Academic Materials} data, including academic papers, journal articles, research reports, and patents, are high-quality texts authored by experts that provide accurate and professional information for pre-training corpora, helping models understand academic terminology and domain-specific knowledge. Common sources like arXiv~\footnote{\hyperlink{https://arxiv.org/}{https://arxiv.org/}}, S2ORC~\autocite{lo2019s2orc}. PubMed Central~\footnote{\hyperlink{https://www.ncbi.nlm.nih.gov/pmc/}{https://www.ncbi.nlm.nih.gov/pmc/}} specifically offers structured content in the medical field. While exclusive academic material corpora are rare, multi-category corpora like The Pile~\autocite{gao2020pile} and RedPajama-V1~\footnote{\hyperlink{https://huggingface.co/datasets/togethercomputer/RedPa jama-Data-1T}{https://huggingface.co/datasets/togethercomputer/RedPa jama-Data-1T}} incorporate a significant proportion of academic texts, including academic material data accounts for 38.1\% and 2.31\% out of 28 billion tokens, respectively.
    \item \textbf{Code} consists of text containing programming languages like Python, Java, and C++, and is crucial for training models to understand code structures and perform tasks such as code comprehension, recommendation, and generation. Key code corpora, including The Stack~\autocite{kocetkov2022stack}, BIGQUERY~\autocite{nijkamp2022codegen}, GitHub, and StackOverflow, provide diverse and high-quality code data that significantly impacts the performance of code models, with recent datasets like phi-1~\autocite{gunasekar2023textbooks} incorporating both curated and AI-generated programming resources.
    \item \textbf{Parallel Corpus} data consists of text pairs in different languages that are translations of each other, which are essential for improving the machine translation and cross-lingual capabilities of LLMs~\autocite{banon2020paracrawl,eisele2010multiun,ziemski2016united}.
    % These corpora are typically collected \textbf{by extracting text from internet resources}, as seen with ParaCrawl~\autocite{banon2020paracrawl} and MTP~\footnote{\hyperlink{https://data.baai.ac.cn/details/BAAI-MTP}{https://data.baai.ac.cn/details/BAAI-MTP}}, or \textbf{by compiling multilingual documents from the United Nations}, such as MultiUN~\autocite{eisele2010multiun} and UNCorpus~\autocite{ziemski2016united}.
    % \item \textbf{Social Media} data consists of user-generated posts, comments, and dialogues from platforms like StackExchange~\footnote{\hyperlink{https://stackexchange.com/}{https://stackexchange.com/}}, Reddit~\footnote{\hyperlink{www.reddit.com}{www.reddit.com}}, and Zhihu~\footnote{\hyperlink{https://www.zhihu.com/}{https://www.zhihu.com/}}, reflecting real-time dynamics and interactions~\autocite{radford2019language,baumgartner2020pushshift}. 
    % Despite containing potentially harmful content, this data is valuable for pre-training LLMs to enhance their conversational abilities, understand social trends, and capture user behavior patterns, with datasets like WebText~\autocite{radford2019language}, OpenWebText~\footnote{\hyperlink{http://Skylion007.github.io/ OpenWebTextCorpus}{http://Skylion007.github.io/ OpenWebTextCorpus}}, and Pushshift Reddit~\autocite{baumgartner2020pushshift} widely used for these purposes.
    \item \textbf{Encyclopedia} data, extracted from sources like Wikipedia and Baidu Baike, is written and edited by experts and community contributors, providing authoritative and reliable content that enhances the knowledge base of LLMs. 
    % Due to its accessibility, multilingual nature, and high textual value, encyclopedia data is frequently included in pre-training corpora to support comprehensive language understanding and knowledge representation.
\end{itemize}

% Multi-category corpora, combining diverse data types, enhance LLMs' generalization abilities and can be used directly for pre-training or by mixing single-category corpora. Examples of English multi-category corpara include RedPajama-V1~\footnote{\hyperlink{https://huggingface.co/datasets/togethercomputer/RedPa jama-Data-1T}{https://huggingface.co/datasets/togethercomputer/RedPa jama-Data-1T}}, which focuses on webpage content; The Pile~\autocite{gao2020pile} and TigerBot\_pretrain\_en~\autocite{chen2023tigerbot}, known for balanced data distributions; Dolma~\autocite{soldaini2024dolma}, with 3T tokens from six domains; and Chinese multi-category corpora like MNBVC~\footnote{\hyperlink{https://github.com/esbatmop/MNBVC}{https://github.com/esbatmop/MNBVC}} and TigerBot\_pretrain\_zh~\autocite{chen2023tigerbot}. Other notable corpora are the bilingual WanJuanText-1.0~\autocite{he2023wanjuan}, multilingual ROOTS~\autocite{laurenccon2022bigscience}, and the ArabicText 2022~\footnote{\hyperlink{https://data.baai.ac.cn/details/ArabicText-2022}{https://data.baai.ac.cn/details/ArabicText-2022}} corpus for Arabic LLMs.

\paragraph{Domain-Specific Pre-Training Corpora}
Domain-Specific Pre-Training Corpora are tailored for specific fields and used in the incremental pre-training phase of LLMs after they have been trained on a general pre-training corpus. These specialized corpora enhance a model's capabilities in specific domains, such as transportation, finance, medicine, law, and mathematics, by building on the general proficiency gained from initial pre-training.
Specifically, in transportation domain, the TransGPT-pt corpus~\footnote{\hyperlink{https://github.com/DUOMO/TransGPT}{https://github.com/DUOMO/TransGPT}} is China's first open-source large-scale transportation model, providing diverse data on transportation literature, technology projects, traffic statistics, engineering, management, and terminology to support research and model development in transportation fields.
% \begin{itemize}
%     \item \textbf{Transportation Domain}: The TransGPT-pt corpus~\footnote{\hyperlink{https://github.com/DUOMO/TransGPT}{https://github.com/DUOMO/TransGPT}} is China's first open-source large-scale transportation model, providing diverse data on transportation literature, technology projects, traffic statistics, engineering, management, and terminology to support research and model development in transportation fields.
%     \item \textbf{Financial Domain}: Financial pre-training corpora like BBT-FinCorpus~\autocite{lu2023bbt}, FinCorpus~\autocite{zhang2023xuanyuan}, FinGLM~\footnote{\hyperlink{https://github.com/MetaGLM/FinGLM}{https://github.com/MetaGLM/FinGLM}}, and TigerBot-earning~\autocite{chen2023tigerbot} focus on topics like financial markets, economics, and investment. These corpora typically include data from financial news, company reports, financial statements, and research papers, which help models learn domain-specific financial knowledge.
%     \item \textbf{Medical Domain}: Corpora in the medical field, such as Medical-pt~\footnote{\hyperlink{https://github.com/ shibing624/MedicalGPT}{https://github.com/ shibing624/MedicalGPT}} and PubMed Central~\footnote{\hyperlink{https://www.ncbi.nlm.nih.gov/pmc/}{https://www.ncbi.nlm.nih.gov/pmc/}}, provide learning materials on diseases, drugs, medical research, and more. The data comes from medical literature, healthcare diagnostic records, case reports, medical news, and textbooks, which are crucial for training models in healthcare-related applications.
%     \item \textbf{Legal Domain}: The TigerBot-law~\autocite{chen2023tigerbot} corpus focuses on legal text data, including 11 categories of Chinese laws and regulations. Text data in this domain comes from legal documents, court cases, law books, legal clauses, and legal news, helping models understand legal concepts and contexts.
%     \item \textbf{Mathematics Domain}: The Proof-Pile-2~\autocite{azerbayev2023llemma} corpus is designed for training mathematical LLMs like Llemma. It contains mathematical code (in 17 programming languages), web data, and papers, which supports advanced mathematical reasoning tasks.
% \end{itemize}

% \paragraph{Preprocessing of Pre-training Data}
% Preprocessing of pre-training data generally consists of five steps: (1) \textbf{Data Collection}. (2) \textbf{Data Filtering}. (3) \textbf{Data Deduplication}. (4) \textbf{Data Standardization}. (5) \textbf{Data Review}.
% \begin{itemize}
%     \item \textbf{Data Collection} includes: 1) Define Data Requirements: Clearly specify data types, languages, domains, sources, and quality standards based on the model’s application needs; 2) Select Data Sources: Choose reliable sources like websites, books, and academic papers, using filters to exclude low-quality content (e.g., CulturaX~\autocite{nguyen2023culturax} corpus); 3) Develop Collection Strategy: Determine the time span, scale, frequency, and methods for collecting diverse and real-time data; 4) Data Crawling and Collection: Use tools like web crawlers and APIs for data retrieval while complying with legal regulations; 5) Data Extraction, Parsing, Encoding, and Language Detection: Extract relevant text (e.g., HTML parsing~\autocite{penedo2023refinedweb,banon2020paracrawl}, PDF text extraction~\autocite{lo2019s2orc}, etc.), detect encoding (e.g., MNBVC~\footnote{\hyperlink{https://github.com/esbatmop/MNBVC}{https://github.com/esbatmop/MNBVC}} corpus), and classify languages (e.g., WanJuanText-1.0~\autocite{he2023wanjuan} using pyclid2~\footnote{\hyperlink{https://pypi.org/pro ject/pycld2/}{https://pypi.org/pro ject/pycld2/}}); 6) Data Backup, Compliance, and Maintenance: Regularly back up data, ensure privacy compliance, and update collection systems to maintain data quality and relevance.
%     \item \textbf{Data Filtering} for pre-training LLMs improves data quality through model-based and heuristic-based methods. \textbf{Model-based methods} train classifiers using high-quality corpora as positive samples and contaminated text as negative samples; for example, WanJuanText-1.0~\autocite{he2023wanjuan} employs models to filter harmful content like obscenity and low-quality data like advertisements. \textbf{Heuristic-based methods} apply rules at the document and sentence levels, such as language filtering (e.g., RefinedWeb~\autocite{penedo2023refinedweb} retains only English, WuDaoCorpora-Text~\autocite{yuan2021wudaocorpora} retains only Chinese), quality metrics like quality filtering scores~\autocite{chen2023tigerbot}, text density~\autocite{yuan2021wudaocorpora,laurenccon2022bigscience,he2023wanjuan,raffel2020exploring,xue2020mt5}, document length~\autocite{zhu2015aligning,he2023wanjuan}, proportion of special characters~\autocite{laurenccon2022bigscience,he2023wanjuan,nguyen2023culturax}, number of short lines~\autocite{nguyen2023culturax}, perplexity scores~\autocite{nguyen2023culturax}, etc. Specific rules are tailored for each corpus, such as excluding non-English or title-less papers in S2ORC~\autocite{lo2019s2orc}, or removing redundant elements like navigation bars~\autocite{penedo2023refinedweb}. Different corpora utilize these techniques to ensure high-quality and relevant data for training.
%     \item \textbf{Data Deduplication} removes duplicate or highly similar texts from a corpus using various methods. TF-IDF (Term Frequency-Inverse Document Frequency) Soft Deduping~\autocite{chen2023tigerbot} calculates the TF-IDF weight for each word to compare text similarities, deleting those above a certain threshold. MinHash~\autocite{penedo2023refinedweb,nguyen2023culturax} and SimHash~\autocite{yuan2021wudaocorpora,abadji2022towards} are computationally efficient methods that estimate similarity by comparing hash values or Hamming distances between text hashes. Other methods include removing duplicates based on repeating sequences of sentences (e.g., CLUECorpus2020~\autocite{xu2020cluecorpus2020}, C4~\autocite{raffel2020exploring}, RefinedWeb~\autocite{penedo2023refinedweb}), URL-based deduplication (CulturaX~\autocite{nguyen2023culturax}), and MinHashLSH combined with n-grams for similarity assessment (WanJuanText-1.0~\autocite{he2023wanjuan}). These approaches help maintain diverse and unique content within corpora.
%     \item \textbf{Data Standardization} involves normalizing and transforming text data to enhance its usability in model training, typically through four steps: 1) Sentence Splitting: MultiUN~\autocite{eisele2010multiun} uses regular expressions for Chinese and NLTK toolkit~\footnote{\hyperlink{https://www.nltk.org/}{https://www.nltk.org/}} for other texts, while CLUECorpus2020~\autocite{xu2020cluecorpus2020} uses PyLTP (Python Language Technology Platform) to separate sentences. 2) Simplified Chinese Conversion: WuDaoCorpora-Text~\autocite{yuan2021wudaocorpora} converts traditional Chinese characters to simplified Chinese. 3) Spelling Correction: Pre-trained models are used to correct spelling errors in the text. 4) Removing Stop Words: High-frequency, low-value words and meaningless spaces in Chinese text are removed~\autocite{yuan2021wudaocorpora,xu2020cluecorpus2020}. These steps ensure that the text is clean, consistent, and ready for effective model training.
%     \item \textbf{Data Review} involves thoroughly documenting preprocessing steps and conducting a manual review to ensure data quality meets expected standards; feedback from this review is used to refine earlier preprocessing steps. This process, as referenced in works like CLUECorpus2020~\autocite{xu2020cluecorpus2020}, can be performed at the end of each preprocessing step for continuous improvement.
% \end{itemize}

\subsubsection{Instruction Fine-tuning Datasets}
    Instruction fine-tuning datasets consist of text pairs with ``instruction inputs'' and ``answer outputs'' designed to help LLMs understand and follow human commands across tasks like classification, summarization, and code generation, while improving their ability to align with human expectations for accurate responses. %These datasets can be 1) built manually, 2) generated using methods like Self-Instruct~\cite{wang2022self}, 3) by collecting and improving existing open source datasets or 4) a combination of the three aforementioned methods, and are categorized as general or domain-specific instruction fine-tuning datasets. 
    
    % Categorizing based on the purpose of instruction fine-tuning follows an evolutionary process. InstructGPT-sft~\autocite{ouyang2022training} organizes instructions into 10 categories, including Generation, Open QA, Brainstorming, Summarization, etc. BELLE\_train\_3.5M\_CN~\footnote{\hyperlink{https://github.com/LianjiaTech/BELLE}{https://github.com/LianjiaTech/BELLE}} expands this by adding Role-playing, Math, Translation, and Code, while removing Chat and Other categories. Firefly~\footnote{\hyperlink{https://github.com/yangjianxin1/Firefly}{https://github.com/yangjianxin1/Firefly}} further refines these categories into 23, with subcategories like story and lyric generation under ``Generation.'' Currently, instructions are broadly grouped into 15 classes: Reasoning, Math, Brainstorming, Closed QA, Open QA, Code, Extraction, Generation, Rewrite, Summarization, Translation, Role-playing, Social Norms, and Others.

\paragraph{General instruction fine-tuning datasets}
General instruction fine-tuning datasets cover various instruction types without domain limitations and are designed to improve LLMs' ability to follow instructions in general tasks. These datasets are built using four main methods: (1) human generation, (2) model construction, (3) collecting and improving existing datasets, or (4) a combination of these approaches.
\begin{itemize}
    \item \textbf{Human Generation (HG)}: Human-generated datasets are manually created by annotators without using existing LLMs, offering advantages such as high quality, interpretability, and flexible control over tasks, but they come with drawbacks like high cost, low efficiency, and potential subjectivity (e.g., Databricks-dolly-15K~\autocite{conover2023free}, OASST1~\autocite{wang2023openchat}, Aya Dataset~\autocite{singh2024aya}, InstructionWild\_v2~\autocite{xue2023instruction}, LCCC~\autocite{wang2020large}). 
    % For example, Databricks-dolly-15K~\autocite{conover2023free} was crafted by Databricks employees, while OASST1~\autocite{wang2023openchat} involved 13.5K volunteers through crowdsourcing. OL-CC~\footnote{\hyperlink{https://data.baai.ac.cn/details/OL-CC}{https://data.baai.ac.cn/details/OL-CC}} is the first open-source Chinese instruction dataset generated via crowdsourcing with 276 volunteers, and the Aya Dataset~\autocite{singh2024aya} is the largest multilingual instruction dataset annotated by 2,997 contributors. Another approach involves scraping real Q\&A data from the web, as seen in InstructionWild\_v2~\autocite{xue2023instruction} and the LCCC~\autocite{wang2020large} dataset, which uses social media conversations.
    \item \textbf{Model Construction (MC)}: Model-generated datasets use LLMs to generate instructional data, offering advantages like abundant data generation and cost-efficiency (e.g., self-Instruct~\autocite{wang2022self}, Alpaca~\autocite{taori2023instruction}, MOSS\_002\_sft\_data~\autocite{sun2023moss}, LMSYS-Chat-1M~\autocite{zheng2023lmsys}, CAMEL~\autocite{li2023camel}, UltraChat~\autocite{ding2023enhancing}). 
    % However, the quality of the content can vary, with issues such as hallucination and bias requiring post-processing. Various methods are used to guide LLMs, including BELLE\_train\_0.5M\_CN~\footnote{\hyperlink{https:// github.com/LianjiaTech/BELLE}{https:// github.com/LianjiaTech/BELLE}} and MOSS\_002\_sft\_data~\autocite{sun2023moss}. Another approach involves using real conversations between humans and LLMs, as in ShareGPT~\footnote{\hyperlink{https://sharegpt.com/}{https://sharegpt.com/}} and LMSYS-Chat-1M~\autocite{zheng2023lmsys}. Additionally, multi-agent LLM dialogue frameworks like CAMEL~\autocite{li2023camel} and UltraChat~\autocite{ding2023enhancing} engage multiple LLMs in role-playing to generate instructional data.
    \item \textbf{Collection and Improvement of Existing Datasets (CI)}: This method integrates and modifies open-source datasets to create comprehensive instruction fine-tuning data, offering advantages like diversity, large scale, and time efficiency (e.g., CrossFit~\autocite{ye2021crossfit}, Flan 2022~\autocite{longpre2023flan}, InstructDial~\autocite{gupta2022instructdial}, OPT-IML Bench~\autocite{iyer2022opt}, SUPER-NATURAL INSTRUCTIONS~\autocite{wang2022super}). 
    % Examples include CrossFit~\autocite{ye2021crossfit}, which compiles 269 NLP datasets across 13 task types~\autocite{wang2022super}, and Flan 2022~\autocite{longpre2023flan}, which aggregates 1836 tasks from various sources. InstructDial~\autocite{gupta2022instructdial} combines 59 open-source dialogue datasets to enhance dialogue-related tasks, while OPT-IML Bench~\autocite{iyer2022opt} merges eight repositories for research on instruction fine-tuning. Though efficient, these datasets require quality and format standardization, as seen in SUPER-NATURAL INSTRUCTIONS~\autocite{wang2022super}, which covers 1616 task datasets in 55 languages. Dataset licenses are also critical to avoid privacy issues.
    \item \textbf{Combination Method}: In constructing instruction fine-tuning datasets, multiple methods are often combined to enhance data quality, leading to four scenarios: HG \& CI (e.g., Firefly~\footnote{\hyperlink{https://github. com/yangjianxin1/Firefly}{https://github. com/yangjianxin1/Firefly}}, LIMA-sft~\autocite{zhou2024lima}), HG \& MC (e.g., InstructGPT-sft~\autocite{ouyang2022training}), CI \& MC (e.g., Alpaca\_GPT4\_data~\autocite{peng2023instruction}, Baize~\autocite{xu2023baize}), and HG \& CI \& MC (e.g., COIG~\autocite{zhang2023chinese}, Aya Collection~\autocite{singh2024aya}, Phoenix-sft-data-v1~\autocite{chen2023phoenix}, TigerBot\_sft\_en \& zh ~\autocite{chen2023tigerbot}). 
    % For HG \& CI, Firefly~\footnote{\hyperlink{https://github. com/yangjianxin1/Firefly}{https://github. com/yangjianxin1/Firefly}} combines collected and manually written instructions for tasks like poetry creation, while LIMA-sft~\autocite{zhou2024lima} manually selects data for quality control. 
    % In HG \& MC, InstructGPT-sft~\autocite{ouyang2022training} uses both manually created and model-generated instructions. For CI \& MC, Alpaca\_GPT4\_data~\autocite{peng2023instruction} uses instructions from Alpaca~\autocite{taori2023instruction} and GPT-4 to generate responses, and Baize~\autocite{xu2023baize} uses datasets to prompt ChatGPT for multi-turn dialogues. 
    % HG \& CI \& MC datasets like COIG~\autocite{zhang2023chinese} use a combination of manual creation, model generation, and improved existing data to cover domains like Chinese exams and value alignment, while Aya Collection~\autocite{singh2024aya} incorporates templated, translated, and human-annotated data. Other examples include Phoenix-sft-data-v1~\autocite{chen2023phoenix} and TigerBot\_sft\_en \& zh ~\autocite{chen2023tigerbot}, which leverage open-source and self-developed data.
\end{itemize}

\paragraph{Domain-specific instruction fine-tuning datasets}
Domain-specific instruction fine-tuning datasets are tailored for particular domains, enhancing a model’s performance in specialized tasks such as transportation, medical, code, legal, and educational fields. Specially, in the transportation domain, TransGPT-sft~\footnote{\hyperlink{https://github.com/DUOMO/TransGPT}{https://github.com/DUOMO/TransGPT}} fine-tunes China's TransGPT traffic model using dialogue-based methods by extracting content from PDFs and Doc files, and generating traffic-related dialogues via LLMs. This approach allows for high performance in transportation-related tasks.

\subsubsection{Preference Datasets}
    Preference datasets evaluate multiple responses to the same instruction, providing feedback through voting, sorting, or scoring methods to capture human or model preferences. These datasets are essential for aligning LLMs with human expectations in three main areas of utility, honesty, and safety~\autocite{zhao2023survey}. Preference data can come from humans, offering real-world insight but with potential subjectivity, or from models, which are more efficient but can introduce biases. A balanced approach, combining both human and model feedback, ensures more effective alignment with human preferences. Preference datasets are categorized based on evaluation methods: voting, sorting, scoring, and other approaches. 

\begin{itemize}
    \item \textbf{Vote}: The voting method for preference datasets involves selecting the better option from two or more answers, offering simplicity and ease of collection, though it lacks granularity (e.g., Chatbot-arena-conversations~\autocite{zheng2023judging}, hh-rlhf~\autocite{bai2022training,perez2022red}, MT-Bench-human-judgments~\autocite{zheng2023judging}, PKU-SafeRLHF~\autocite{ji2024beavertails}, CValues~\autocite{xu2023cvalues}). 
    % Examples include Chatbot\_arena\_conversations~\autocite{zheng2023judging}, where human judges select the better answer from two models in multiple languages, and hh-rlhf dataset~\autocite{bai2022training,perez2022red}, where crowdworkers choose the more useful and honest response. MT-Bench\_human\_judgments~\autocite{zheng2023judging} uses graduate students to compare model responses, and PKU-SafeRLHF~\autocite{ji2024beavertails} focuses on safety and usefulness in Q\&A formats. A model-based voting example is CValues~\autocite{xu2023cvalues}, where models evaluate responses based on safety and social norms.
    \item \textbf{Sort}: The sorting method ranks multiple responses to a question based on predefined criteria, offering detailed information on relative preferences but requiring more effort to collect and process (e.g., OASST1 dataset~\autocite{wang2023openchat}). 
    % OASST1\_pairwise\_rlhf\_reward~\footnote{\hyperlink{https://huggingface.co/datasets/tasksource/oasst1 pairwise rlhf reward}{https://huggingface.co/datasets/tasksource/oasst1 pairwise rlhf reward}} is a key dataset that uses this approach, building on the OASST1 dataset~\autocite{wang2023openchat}, which includes human-generated dialogues rated for quality. These ratings allow for the sorting of responses according to human preferences, providing valuable data for RLHF (Reinforcement Learning from Human Feedback). Although sorting offers granular insights, standardizing the criteria across tasks is essential for consistency.
    \item \textbf{Score}: The scoring method assigns numerical values to responses, offering a more flexible and nuanced way to reflect human preferences (e.g., Stack-Exchange-Preferences~\autocite{askell2021general}, Summarize\_from\_Feedback~\autocite{stiennon2020learning}, WebGPT~\autocite{nakano2021webgpt}, Alpaca\_comparison\_data~\autocite{peng2023instruction}, Stable\_Alignment~\autocite{liu2023training}, UltraFeedback~\autocite{cui2023ultrafeedback}). 
    % Stack-Exchange-Preferences~\autocite{askell2021general} derives scores from StackOverflow answers based on likes and acceptance by the question asker. In Summarize\_from\_Feedback~\autocite{stiennon2020learning}, responses are rated using the Likert scale, while WebGPT~\autocite{nakano2021webgpt} provides human-assigned scores for two model answers to indicate preference. Models can also be used for scoring, as seen in Alpaca\_comparison\_data~\autocite{peng2023instruction}, where GPT-4 scores responses, and Stable\_Alignment~\autocite{liu2023training}, which scores model-generated responses from simulated social interactions. UltraFeedback~\autocite{cui2023ultrafeedback} enriches this process by scoring responses across four dimensions with detailed textual explanations.
    \item \textbf{Other}: In addition to voting, sorting, and scoring methods, some preference datasets use alternative evaluation methods (e.g., Medical-rlhf~\footnote{\hyperlink{https://github.com/ shibing624/MedicalGPT}{https://github.com/ shibing624/MedicalGPT}}, PRM800K~\autocite{lightman2023let}). 
    % Medical-rlhf~\footnote{\hyperlink{https://github.com/ shibing624/MedicalGPT}{https://github.com/ shibing624/MedicalGPT}} is a Chinese dataset for aligning medical models, containing 4K examples with comparisons between professional doctor replies and model-generated responses. Though effective, its small scale and binary quality assessment are limitations. PRM800K~\autocite{lightman2023let} focuses on mathematical problem-solving, with 102K model-generated solutions labeled by human annotators. This dataset provides step-level feedback for 12K problems, offering an alignment signal by assessing the correctness of each solution step, helping models in the CoT (Chain-of-Thought) process for mathematics.
\end{itemize}


\subsubsection{Evaluation Datasets}

Guo et al.~\autocite{guo2023evaluating} classifies LLM evaluations into five key categories: knowledge and capability evaluation, alignment evaluation, safety evaluation, specialized LLM evaluation, and evaluation organization. Among the many evaluation datasets, these can be grouped into various domains. Here, the focus is on key evaluation domains such as General, Exam, Natural Language Understanding (NLU), Reasoning, Code, Out-of-Distribution (OOD), Multitask, Multilingual and others.

\begin{itemize}
    \item \textbf{General}: General evaluation datasets focus on assessing LLMs in two main areas: their versatility across multiple domains and their ability to follow complex instructions (e.g., AlpacaEval~\autocite{dubois2024alpacafarm}, BayLing-80~\autocite{zhang2023bayling}, BELLE\_eval~\autocite{ji2023exploring}, MT-Bench~\autocite{zheng2023judging}, SuperCLUE~\autocite{xu2023superclue}, CELLO~\autocite{he2024can}). 
    % Vicuna Evaluation assesses models in nine categories, using GPT-4 for judging output quality, while AlpacaEval~\autocite{dubois2024alpacafarm} expands this to cover a broader range of open-ended questions. BayLing-80~\autocite{zhang2023bayling} evaluates conversational abilities in both Chinese and English, and BELLE\_eval~\autocite{ji2023exploring} and MT-Bench~\autocite{zheng2023judging} assess general performance in Chinese and English scenarios, respectively. Though these datasets are relatively small, with under 1,000 instructions, SuperCLUE~\autocite{xu2023superclue} offers a larger-scale benchmark for Chinese LLMs with tasks like multiturn Q\&A and multiple-choice, updated monthly. In terms of following instructions, CELLO~\autocite{he2024can} stands out by evaluating models on their ability to handle complex tasks and inputs, complementing the general instruction evaluations in other datasets.
    % \item \textbf{Exam}: Examination evaluation datasets focus on testing LLMs' ability to answer exam-style questions from various nations, simulating the role of candidates in responding to these queries. GAOKAO-Bench~\autocite{zhang2023evaluating} uses China's Gaokao exam to assess LLMs' proficiency across 10 subjects. AGIEval~\autocite{zhong2023agieval} broadens this scope by including 20 official exams like Gaokao, the U.S. SAT, bar exams, and civil service exams, targeting human-centric tasks. M3Exam~\autocite{zhang2023m3exam} incorporates multi-modal, multi-lingual, and multi-tiered multiple-choice questions, drawing from primary to high school exams in nine countries with diverse languages. These datasets evaluate the LLMs' understanding of question intent and domain-specific knowledge.
    % \item \textbf{NLU}: Natural Language Understanding (NLU) evaluation datasets assess LLMs' capabilities across a range of tasks, from basic grammar comprehension to advanced semantic reasoning. MCTS~\autocite{chong2023mcts} is a key dataset for Chinese text simplification, while RAFT~\autocite{alex2021raft} benchmarks text classification. GLUE~\autocite{wang2018glue} covers nine English NLU tasks, including sentiment analysis and textual entailment, with SuperGLUE~\autocite{wang2019superglue} increasing task difficulty. In Chinese, CLUE~\autocite{xu2020clue} mirrors GLUE with nine tasks like semantic matching and reading comprehension, while CUGE~\autocite{yao2021cuge} evaluates LLMs using 21 sub-datasets across various tasks. SentEval~\autocite{conneau2018senteval} also aggregates datasets for 21 NLU sub-tasks.
    \item \textbf{Reasoning}: Reasoning evaluation datasets test LLMs' abilities in tasks involving logical reasoning and inference (e.g., Chain-of-Thought Hub~\autocite{fu2023chain}, Choice-75~\autocite{hou2023choice}, NeuLR~\autocite{xu2023large}, TabMWP~\autocite{lu2022dynamic}, LILA~\autocite{mishra2022lila}, miniF2F\_v1~\autocite{zheng2021minif2f}). 
    % Chain-of-Thought Hub~\autocite{fu2023chain} evaluates multi-step reasoning using few-shot prompting across domains like math, science, and symbols. Choice-75~\autocite{hou2023choice} assesses decision-making reasoning by asking LLMs to select appropriate solutions in various scenarios. NeuLR~\autocite{xu2023large} focuses on deductive, inductive, and abductive reasoning. Mathematical reasoning is tested in datasets like TabMWP~\autocite{lu2022dynamic}, which involves table-based Q\&A and math problems, LILA~\autocite{mishra2022lila}, a comprehensive math reasoning benchmark, and miniF2F\_v1~\autocite{zheng2021minif2f}, which includes Olympiad-level math problems. These datasets cover a range of reasoning tasks, including multi-step, decision, deductive, and mathematical reasoning.
    \item \textbf{Code}: Coding evaluation datasets test LLMs' proficiency in programming tasks, such as code interpretation, generation, correction, and optimization. 
    These datasets are divided into two types: single-task ((e.g., APPS~\autocite{hendrycks2021measuring}, DS-1000~\autocite{lai2023ds}, HumanEval~\autocite{chen2021evaluating}, MTPB~\autocite{nijkamp2022codegen}, ODEX~\autocite{wang2022execution}, BIRD~\autocite{li2024can}, Spider~\autocite{yu2018spider})) and multitask evaluations (e.g., CodeXGLUE~\autocite{lu2021codexglue}, HumanEvalPack~\autocite{muennighoff2023octopack}). 
    % APPS~\autocite{hendrycks2021measuring} focuses on Python code generation, while DS-1000~\autocite{lai2023ds} targets data science tasks, and HumanEval~\autocite{chen2021evaluating} assesses manually written programming problems to avoid data leakage. MTPB~\autocite{nijkamp2022codegen} evaluates stepwise code generation, and ODEX~\autocite{wang2022execution} tests multilingual code generation abilities. BIRD~\autocite{li2024can} benchmarks text-to-SQL tasks, bridging the gap between academia and real-world applications, compared to earlier datasets like Spider~\autocite{yu2018spider}. In multitask evaluations, CodeXGLUE~\autocite{lu2021codexglue} categorizes code tasks into four types, while HumanEvalPack~\autocite{muennighoff2023octopack} extends HumanEval~\autocite{chen2021evaluating} to include six languages and tasks like code fixing and comment generation.
    % \item \textbf{OOD}: Out-of-distribution (OOD) evaluation datasets test LLMs' ability to handle tasks they haven't seen during fine-tuning, focusing on their robustness. BOSS~\autocite{yuan2023revisiting} evaluates OOD performance across 5 tasks and 20 sub-datasets, assessing how well LLMs generalize to new tasks. GLUE-X~\autocite{yang2022glue} similarly measures OOD performance, providing insights into how models handle unseen tasks. These datasets are crucial for evaluating the robustness of LLMs in real-world scenarios.
    % \item \textbf{Multitask}: Multitask evaluation datasets assess LLMs' comprehensive capabilities across a wide range of tasks and domains. In English, DecaNLP~\autocite{mccann2018natural} transforms 10 distinct task datasets into a Q\&A format, while LMentry~\autocite{efrat2022lmentry} provides a quick "unit test" for 25 simpler task types. BIG-Bench~\autocite{srivastava2022beyond} covers 95 task types across 204 tasks, including topics like common-sense reasoning and social biases, with BBH~\autocite{suzgun2022challenging} focusing on 23 particularly challenging tasks. HELM~\autocite{liang2022holistic} offers a comprehensive evaluation system with 73 scenarios and 65 metrics. In the Chinese domain, CLEVA~\autocite{li2023cleva} features 31 tasks with 370K samples, and FlagEval~\footnote{\hyperlink{https://github.com/FlagOpen/FlagEval}{https://github.com/FlagOpen/FlagEval}} evaluates models in both Chinese and English across over 600 sub-dimensions. LLMEVAL-1~\footnote{\hyperlink{https: //github.com/llmeval/llmeval-1}{https: //github.com/llmeval/llmeval-1}} and CLiB~\footnote{\hyperlink{https://github.com/jeinlee1991/chinese-llm-benchmark}{https://github.com/jeinlee1991/chinese-llm-benchmark}} provide thorough assessments of Chinese LLMs like GPT-4 and ERNIE Bot.
    % \item \textbf{Multilingual}: Multilingual evaluation datasets test LLMs' abilities in cross-lingual tasks, covering multiple languages and linguistic challenges. XNLI~\autocite{conneau2018xnli} focuses on low-resource language transfer and cross-lingual sentence classification across 15 languages, including English, French, and Chinese. XTREME~\autocite{hu2020xtreme} broadens this with 40 languages across 12 language families, assessing LLMs on four NLP tasks. These datasets extend traditional NLP tasks to include greater language diversity while maintaining moderate difficulty, requiring extensive linguistic knowledge from models.
    \item \textbf{Others}: This section includes several subject-specific evaluation datasets across various academic, professional, and specialized domains (e.g., C-CLUE~\footnote{\hyperlink{https://github.com/jizijing/C-CLUE}{https://github.com/jizijing/C-CLUE}}, MMCU~\autocite{zeng2023measuring}, SCIBENCH~\autocite{wang2023scibench}, BBF-CFLEB~\autocite{lu2023bbt}, FLUE~\autocite{shah2022flue}, SafetyBench~\autocite{zhang2023safetybench}, LongBench~\autocite{bai2023longbench}, API-Bank~\autocite{li2023api}). 
    % For example, C-CLUE~\footnote{\hyperlink{https://github.com/jizijing/C-CLUE}{https://github.com/jizijing/C-CLUE}} assesses classical Chinese language comprehension, focusing on tasks like named entity recognition (NER) and relation extraction (RE), while MMCU~\autocite{zeng2023measuring} evaluates disciplines such as medicine, law, psychology, and education in Chinese semantic comprehension. In mathematics and science, SCIBENCH~\autocite{wang2023scibench} tests LLMs' abilities with university-level questions in physics, chemistry, and math. In finance, BBF-CFLEB~\autocite{lu2023bbt} assesses LLMs in financial text processing and financial tasks, while FLUE~\autocite{shah2022flue} is an English benchmark for financial NLP tasks. SafetyBench~\autocite{zhang2023safetybench} evaluates LLM safety in generating responses across multiple dimensions like ethics, bias, and toxicity, ensuring outputs align with societal norms. For long-text evaluation, LongBench~\autocite{bai2023longbench} assesses LLMs' ability to process and generate long texts, supporting both English and Chinese tasks. API-Bank~\autocite{li2023api} evaluates LLMs' proficiency in using real-world APIs, simulating tool invocation tasks within conversational contexts.
\end{itemize}

\textbf{Evaluation methods} are divided into three categories: code evaluation, human evaluation, and model evaluation. Both code and model evaluations are automated, involving minimal human intervention, and are therefore classified as automated evaluation methods. In contrast, human evaluation is a non-automated approach, relying on direct human input and judgment.

\begin{itemize}
    \item \textbf{Code evaluation} extracts responses from LLMs and uses predefined metrics like accuracy, F1 score, BLEU~\autocite{papineni2002bleu}, ROUGE~\autocite{lin2004rouge}, Exact Match, and Pearson correlation to assess their performance. For instance, accuracy is used in classification tasks, while BLEU evaluates translation quality. This method, ideal for objective and straightforward subjective tasks, is less effective for open-ended questions like generation and brainstorming. Some datasets also provide custom calculation methods and code for direct evaluation.
    \item \textbf{Human evaluation} involves assessing LLM outputs by crowdsourced individuals, trained volunteers, or experts, using methods like quality scoring (e.g., QizhenGPT\_eval~\footnote{\hyperlink{https://github.com/CMKRG/QiZhenGPT/tree/main/data/eval}{https://github.com/CMKRG/QiZhenGPT/tree/main/data/eval}}, CLiB~\footnote{\hyperlink{https://github.com/jeinlee1991/chinese-llm-benchmark}{https://github.com/jeinlee1991/chinese-llm-benchmark}}) and quality comparison~\autocite{xu2023superclue}. While versatile for open-ended or complex tasks, it is limited by high costs, significant resource demands, and potential subjective bias.
    \item \textbf{Model evaluation} introduces a new approach by combining questions, reference answers, and evaluation criteria into an optimal prompt, then inputting it to LLMs for evaluation~\autocite{ji2023exploring,zheng2023judging,zhang2023bayling}. This method reduces manual effort and speeds up evaluation but relies heavily on LLM performance, which may not fully align with human judgments.
\end{itemize}






